Jeu de taquin forests and the inverse infinite RSK correspondence

The Plancherel-random infinite Young tableau arises from applying the infinite Robinson-Schensted-Knuth (RSK) correspondence to a sequence of i.i.d. random variables distributed uniformly on the unit interval [0,1]. Building on the isomorphism of dynamical systems established in prior work, we provide an explicit geometric characterization of the inverse map. Our approach makes use of a previously unexplored structure, the jeu de taquin forest on the infinite tableau, where edges connect boxes according to local comparison rules. We prove that each tree in this forest almost surely extends toward infinity with a well-defined asymptotic direction, establishing a canonical bijection between trees and values in the i.i.d. input sequence. The ordering is recovered through tree lifetimes under iterated jeu de taquin transformations.

==> figures/_boundary-box-defs.tex <==
% Shared definitions for the two panels of fig:boundary-boxes
% (FIGURE-boundary_box-before.tex and FIGURE-boundary_box-after.tex).
% Pure macro definitions, meant to be \input by each panel subfile.

% Colours from the ColorBrewer Paired palette, matching \cref{fig:jdt-slide}.
% Chosen to stay legible on a black-and-white printer: the origin tree is a
% solid light blue, while the neighbouring tree is a pale yellow overlaid
% with NE diagonal stripes, so the two regions differ by texture (not just
% hue) and remain distinct in grayscale.
\tikzset{
	inside/.style={fill=Paired-A},
	outside/.style={fill=Paired-K},
	stripes/.style={pattern={Lines[angle=45,distance=1.4mm,
		line width=0.5pt]}, pattern color=Paired-H},
	edge/.style={very thick,->},
	edge changed/.style={line width=2.5,->,red},
	jdt path/.style={line width=8pt, blue, opacity=0.75,
		line cap=round},
	highlight box/.style={draw=red, very thick,
		minimum size=0.6cm, inner sep=0pt},
	axis label/.style={font=\footnotesize}
}

% The neighbouring tree (\texttt{outside}) is painted as a solid pale-yellow
% background with the diagonal stripe pattern overlaid on top.
\newcommand{\filloutside}[1]{%
	\fill[outside] #1;
	\fill[stripes] #1;
}

% Boundary box at column x, row y (centre of the window). Flip box to
% its west (column x-1, row y); the box that does not belong to the
% origin tree to the north-west (column x-1, row y+1). The grid is
% drawn larger than the clipping window so that the lattice is seen
% to continue beyond the depicted region.
%
% The single argument selects the panel state:
%   a -- before the slide: the flip box and the boundary box both
%        belong to the origin tree (light blue), and the thick line marks
%        the part of the tree boundary between them.
%   b -- after the slide: the origin tree at the origin has dissolved.
%        The flip box now belongs to the same tree as the box to its
%        north (striped pale yellow), the boundary box's tree membership
%        is unknown (left unpainted), and the dissolved boundary line is
%        gone.
\newcommand{\boundaryboxcontent}[1]{%
	% Origin tree (light blue) and the neighbouring tree (striped yellow).
	\if a#1%
		\fill[inside] (0,0) rectangle +(1,1);% flip box (x-1,y)
		\fill[inside] (1,0) rectangle +(1,1);% boundary box (x,y)
	\else
		\filloutside{(0,0) rectangle +(1,1)}% flip box joins tree above
		% boundary box (x,y) left unpainted: membership unknown.
	\fi
	\filloutside{(0,1) rectangle +(1,1)}% empty box (x-1,y+1)
	\draw[gray,thick] (-2,-3) grid (5,4);
	% Part of the boundary of the origin tree (only before the slide;
	% after the slide it has dissolved at this place).
	\if a#1%
		\draw[line width=5pt] (0,1) -- (1,1);
	\fi
	% The jeu de taquin path through the boundary box, drawn as a
	% vague smooth snake running from the (x-1,y-1) corner to the
	% (x+1,y+1) corner: entry (W/S) and exit (N/E) are undetermined.
	\draw[jdt path] (0.45,-0.4)
		.. controls (1.45,-0.1) and (0.85,0.55) .. (1.5,0.5)
		.. controls (2.2,0.45) and (1.55,1.1) .. (2.5,1.35);
	% Marks: outside box, flip box (red square), boundary box (cross).
	\node at (0.5,1.5) {$\emptyset$};
	\node[highlight box] at (0.5,0.5) {};
	\draw[line width=5pt,black] (1.5,0.5) +(0.25,0.25) -- +(-0.25,-0.25)
		+(0.25,-0.25) -- +(-0.25,0.25);
}

% Column headers (x-axis) and row headers (y-axis), drawn in the clean
% margin outside the clipped lattice window.
\newcommand{\boundaryboxlabels}{%
	\node[axis label,anchor=north] at (0.5,-1.55) {$x-1$};
	\node[axis label,anchor=north] at (1.5,-1.55) {$x$};
	\node[axis label,anchor=north] at (2.5,-1.55) {$x+1$};
	\node[axis label,anchor=east] at (-0.6,-0.5) {$y-1$};
	\node[axis label,anchor=east] at (-0.6,0.5) {$y$};
	\node[axis label,anchor=east] at (-0.6,1.5) {$y+1$};
}


==> figures/autogenerated/_common_color_scheme.tex <==
% Generated by 02_generate_color_scheme.ipynb

\colorlet{vertex-}{Paired-K}
\colorlet{vertex-L}{Paired-A}
\colorlet{vertex-R}{Paired-H}
\colorlet{vertex-RR}{Paired-J}
\colorlet{vertex-LR}{Paired-F}
\colorlet{vertex-LRL}{white}
\colorlet{vertex-LRR}{Paired-C}
\colorlet{vertex-LL}{Paired-B}
\colorlet{vertex-LRRL}{Paired-J}
\colorlet{vertex-LRRLL}{Paired-L}
\colorlet{vertex-LRRRR}{Paired-D}
\colorlet{vertex-RL}{Paired-I}
\colorlet{vertex-LLL}{Paired-G}
\colorlet{vertex-RLL}{Paired-E}
\colorlet{vertex-RRL}{Paired-G}
\colorlet{vertex-LLR}{Paired-D}
\colorlet{vertex-RLR}{Paired-B}
\colorlet{vertex-RRR}{white}
\colorlet{vertex-LRLR}{Paired-G}
\colorlet{vertex-RLLL}{Paired-G}
\colorlet{vertex-LLRR}{Paired-E}
\colorlet{vertex-RRLL}{white}
\colorlet{vertex-RRLR}{Paired-E}
\colorlet{vertex-RLRL}{white}
\colorlet{vertex-RRRR}{Paired-D}
\colorlet{vertex-LLLR}{Paired-I}
\colorlet{vertex-LLLL}{Paired-J}
\colorlet{vertex-LRLL}{Paired-H}
\colorlet{vertex-RLRR}{Paired-D}
\colorlet{vertex-LRRR}{Paired-B}
\colorlet{vertex-RRRL}{Paired-C}
\colorlet{vertex-LLRL}{Paired-C}
\colorlet{vertex-RLLR}{Paired-D}
\colorlet{vertex-LRRRL}{Paired-G}
\colorlet{vertex-LLLLR}{Paired-H}
\colorlet{vertex-RLLLL}{Paired-H}
\colorlet{vertex-RLRRL}{Paired-C}
\colorlet{vertex-RRRLR}{Paired-F}
\colorlet{vertex-RLLLR}{Paired-J}
\colorlet{vertex-LLRRR}{Paired-G}
\colorlet{vertex-RLRLR}{Paired-F}
\colorlet{vertex-RRRRR}{Paired-A}
\colorlet{vertex-RRLLL}{Paired-E}
\colorlet{vertex-RRLRL}{Paired-F}
\colorlet{vertex-LRLRL}{Paired-I}
\colorlet{vertex-RLRRR}{Paired-A}
\colorlet{vertex-RLLRR}{Paired-A}
\colorlet{vertex-RRRLL}{Paired-A}
\colorlet{vertex-LLLRL}{Paired-E}
\colorlet{vertex-LRRLR}{Paired-E}
\colorlet{vertex-RLRLL}{Paired-J}
\colorlet{vertex-LLRRL}{Paired-J}
\colorlet{vertex-LRLLR}{Paired-E}
\colorlet{vertex-RLLRL}{white}
\colorlet{vertex-LLLLL}{white}
\colorlet{vertex-LLRLL}{white}
\colorlet{vertex-LRLLL}{Paired-K}
\colorlet{vertex-LRLRR}{Paired-D}
\colorlet{vertex-LLLRR}{Paired-H}
\colorlet{vertex-RRRRL}{Paired-B}
\colorlet{vertex-RRLRR}{Paired-I}
\colorlet{vertex-LLRLR}{Paired-H}
\colorlet{vertex-RRLLR}{Paired-A}
\colorlet{vertex-LLRLLL}{Paired-F}
\colorlet{vertex-RRLRLR}{Paired-D}
\colorlet{vertex-RRLRRR}{Paired-K}
\colorlet{vertex-LRLRRR}{Paired-A}
\colorlet{vertex-LRLRLL}{Paired-J}
\colorlet{vertex-LRRRLR}{white}
\colorlet{vertex-LLRRRL}{Paired-I}
\colorlet{vertex-RLLLLR}{white}
\colorlet{vertex-LLRRRR}{Paired-B}
\colorlet{vertex-RRRLRL}{Paired-K}
\colorlet{vertex-RRRLLL}{Paired-F}
\colorlet{vertex-LRRRRL}{Paired-A}
\colorlet{vertex-LLLLLL}{Paired-K}
\colorlet{vertex-RLRLLR}{Paired-G}
\colorlet{vertex-LLLRLR}{Paired-K}
\colorlet{vertex-LRLRRL}{Paired-B}
\colorlet{vertex-RLLLRR}{Paired-C}
\colorlet{vertex-RLLLLL}{Paired-I}
\colorlet{vertex-RLLRLR}{Paired-F}
\colorlet{vertex-LLLLRR}{Paired-K}
\colorlet{vertex-RRRLLR}{Paired-I}
\colorlet{vertex-LLRLLR}{Paired-K}
\colorlet{vertex-LLRRLL}{Paired-F}
\colorlet{vertex-RLRLLL}{Paired-H}
\colorlet{vertex-LLLRLL}{Paired-F}
\colorlet{vertex-LLLRRR}{Paired-J}
\colorlet{vertex-RRLRRL}{Paired-B}
\colorlet{vertex-RRRLRR}{Paired-E}
\colorlet{vertex-RRLLLR}{Paired-C}
\colorlet{vertex-RLRRRR}{Paired-K}
\colorlet{vertex-RLRRLL}{Paired-G}
\colorlet{vertex-RLLRRL}{Paired-C}
\colorlet{vertex-LRLLLR}{Paired-C}
\colorlet{vertex-RRLLLL}{Paired-J}
\colorlet{vertex-LRLLLL}{Paired-F}
\colorlet{vertex-LLRLRL}{Paired-F}
\colorlet{vertex-LLRLRR}{Paired-I}
\colorlet{vertex-RRRRLR}{Paired-K}
\colorlet{vertex-LRRRRR}{Paired-F}
\colorlet{vertex-LLLRRL}{Paired-F}
\colorlet{vertex-RLRRLR}{Paired-K}
\colorlet{vertex-RRLLRR}{Paired-K}
\colorlet{vertex-LRRLLR}{Paired-I}
\colorlet{vertex-LRLRLR}{Paired-E}
\colorlet{vertex-LRLLRL}{Paired-J}
\colorlet{vertex-LRLLRR}{Paired-B}
\colorlet{vertex-LLLLLR}{Paired-C}
\colorlet{vertex-LRRRLL}{Paired-H}
\colorlet{vertex-RRLLRL}{Paired-F}
\colorlet{vertex-RRLRLL}{Paired-C}
\colorlet{vertex-LLRRLR}{Paired-C}
\colorlet{vertex-LRRLLL}{Paired-K}
\colorlet{vertex-LLLLRL}{Paired-D}
\colorlet{vertex-RLRRRL}{Paired-E}
\colorlet{vertex-RRRRLL}{Paired-I}
\colorlet{vertex-RLLLRL}{Paired-B}
\colorlet{vertex-RLLRRR}{Paired-K}
\colorlet{vertex-RLLRLL}{Paired-H}
\colorlet{vertex-LLRLRRR}{Paired-B}
\colorlet{vertex-RLLLLLR}{Paired-J}
\colorlet{vertex-LRRRLLR}{Paired-I}
\colorlet{vertex-LRRRLLL}{Paired-K}
\colorlet{vertex-RLRRLRR}{Paired-F}
\colorlet{vertex-RRLRRLR}{Paired-H}
\colorlet{vertex-LRLRRLR}{Paired-H}
\colorlet{vertex-RRLLLRR}{Paired-D}
\colorlet{vertex-RLRLLRL}{Paired-C}
\colorlet{vertex-LRLLLLR}{Paired-I}
\colorlet{vertex-LRRRRLL}{Paired-I}
\colorlet{vertex-RLLLLLL}{Paired-E}
\colorlet{vertex-LRLRRRR}{white}
\colorlet{vertex-RRLRLRL}{Paired-K}
\colorlet{vertex-LLRLLRL}{Paired-E}
\colorlet{vertex-LRLLLRR}{Paired-D}
\colorlet{vertex-LLLLLRL}{Paired-A}
\colorlet{vertex-LRRRLRR}{Paired-J}
\colorlet{vertex-LLLRRLR}{Paired-K}
\colorlet{vertex-LRLRLLR}{Paired-C}
\colorlet{vertex-LRRRLRL}{Paired-A}
\colorlet{vertex-LRLLRRR}{Paired-A}
\colorlet{vertex-LLRLLRR}{Paired-G}
\colorlet{vertex-RLRRLLR}{Paired-J}
\colorlet{vertex-LLRLLLR}{Paired-A}
\colorlet{vertex-RRLRLLR}{Paired-B}
\colorlet{vertex-LLRRRRL}{Paired-C}
\colorlet{vertex-LLLRLLR}{white}
\colorlet{vertex-LRLLLRL}{Paired-J}
\colorlet{vertex-RLRRLRL}{Paired-E}
\colorlet{vertex-LLLLRLL}{Paired-F}
\colorlet{vertex-RLLLRLR}{Paired-F}
\colorlet{vertex-RLLRLLL}{Paired-I}
\colorlet{vertex-LRRRRRR}{Paired-C}
\colorlet{vertex-LLLLRLR}{Paired-A}
\colorlet{vertex-LRLLRLL}{Paired-I}
\colorlet{vertex-LRLLRLR}{Paired-D}
\colorlet{vertex-LRLLRRL}{Paired-C}
\colorlet{vertex-RLRLLRR}{Paired-A}
\colorlet{vertex-RRLRLRR}{Paired-H}
\colorlet{vertex-LRLRLRR}{Paired-H}
\colorlet{vertex-LLRRRRR}{Paired-D}
\colorlet{vertex-LLLLRRL}{Paired-C}
\colorlet{vertex-LLLRLLL}{Paired-B}
\colorlet{vertex-LLLLRRR}{white}
\colorlet{vertex-RLRLLLR}{Paired-A}
\colorlet{vertex-LRLLLLL}{white}
\colorlet{vertex-LRLRLRL}{Paired-K}
\colorlet{vertex-RRLRRLL}{Paired-C}
\colorlet{vertex-LRRRRRL}{Paired-J}
\colorlet{vertex-RRLLLRL}{Paired-F}
\colorlet{vertex-RLRRRRL}{Paired-I}
\colorlet{vertex-LLLRRRR}{Paired-G}
\colorlet{vertex-RLLLRLL}{Paired-I}
\colorlet{vertex-LLRLRRL}{Paired-G}
\colorlet{vertex-RLRRLLL}{Paired-H}
\colorlet{vertex-LLRLLLL}{Paired-D}
\colorlet{vertex-LLLLLRR}{Paired-K}
\colorlet{vertex-LLLRRRL}{white}
\colorlet{vertex-RLLRLRR}{Paired-G}
\colorlet{vertex-LRLRRLL}{Paired-K}
\colorlet{vertex-RLRLLLL}{Paired-B}
\colorlet{vertex-LRRRRLR}{white}
\colorlet{vertex-LLRRLLL}{Paired-A}
\colorlet{vertex-RLLRLLR}{Paired-B}
\colorlet{vertex-LLLRLRR}{Paired-J}
\colorlet{vertex-LRLRLLL}{Paired-F}
\colorlet{vertex-LLLRLRL}{Paired-C}
\colorlet{vertex-RLLRLRL}{Paired-C}
\colorlet{vertex-RLRRRRR}{Paired-B}
\colorlet{vertex-LRLRRRL}{Paired-E}
\colorlet{vertex-LLRRLLR}{white}
\colorlet{vertex-LLLRRLL}{Paired-D}
\colorlet{vertex-RRLRLLL}{Paired-J}
\colorlet{vertex-RLLLLLLR}{white}
\colorlet{vertex-LRRRLLLR}{Paired-D}
\colorlet{vertex-LLLLRRRL}{Paired-A}
\colorlet{vertex-LRRRRRLL}{Paired-E}
\colorlet{vertex-RRLRLLLR}{Paired-I}
\colorlet{vertex-LLLRLLLL}{Paired-I}
\colorlet{vertex-LLLRLLRL}{Paired-A}
\colorlet{vertex-RRLRLLLL}{Paired-F}
\colorlet{vertex-LRRRRLLR}{Paired-H}
\colorlet{vertex-LRLLRRLL}{Paired-G}
\colorlet{vertex-LLLRLRLR}{Paired-A}
\colorlet{vertex-LRLLRRRL}{Paired-K}
\colorlet{vertex-LRLLRRLR}{Paired-D}
\colorlet{vertex-RLLRLRRL}{Paired-J}
\colorlet{vertex-RLLLRLRR}{Paired-A}
\colorlet{vertex-RRLRRLLL}{Paired-J}
\colorlet{vertex-LRRRRRRL}{white}
\colorlet{vertex-RLRRLLLL}{Paired-J}
\colorlet{vertex-RLLLLLRL}{Paired-B}
\colorlet{vertex-LLLLRLRL}{Paired-E}
\colorlet{vertex-RRLRRLLR}{Paired-A}
\colorlet{vertex-RLRLLLLL}{white}
\colorlet{vertex-RRLRLRLR}{Paired-A}
\colorlet{vertex-LLRLLRLL}{Paired-D}
\colorlet{vertex-LLLLRRRR}{Paired-J}
\colorlet{vertex-LLLLRLLR}{Paired-I}
\colorlet{vertex-LLLRLRLL}{Paired-D}
\colorlet{vertex-LRLRRLLL}{Paired-F}
\colorlet{vertex-LLRLLRLR}{Paired-J}
\colorlet{vertex-LRLRLRLL}{Paired-D}
\colorlet{vertex-RLRRLRLL}{Paired-A}
\colorlet{vertex-LLLRRRLR}{Paired-E}
\colorlet{vertex-RLLRLRRR}{Paired-E}
\colorlet{vertex-RLRRLLLR}{Paired-A}
\colorlet{vertex-RLRLLLLR}{Paired-F}
\colorlet{vertex-RLLRLLLR}{Paired-A}
\colorlet{vertex-LRLRRLLR}{Paired-J}
\colorlet{vertex-RLLRLLRR}{Paired-K}
\colorlet{vertex-RLLRLRLR}{Paired-K}
\colorlet{vertex-LRRRRRLR}{Paired-A}
\colorlet{vertex-LLLRLRRR}{Paired-G}
\colorlet{vertex-RLLLLLLL}{Paired-H}
\colorlet{vertex-LRLLRLLL}{white}
\colorlet{vertex-LLLRRLLL}{Paired-B}
\colorlet{vertex-LLLRRRLL}{Paired-C}
\colorlet{vertex-LRLRLRLR}{Paired-A}
\colorlet{vertex-LRRRRLRL}{Paired-E}
\colorlet{vertex-LRLLRRRR}{Paired-H}
\colorlet{vertex-RLRLLLRL}{Paired-C}
\colorlet{vertex-LLLRLRRL}{Paired-D}
\colorlet{vertex-RLLLRLLL}{Paired-E}
\colorlet{vertex-LLLLRLLL}{Paired-B}
\colorlet{vertex-LLRRLLLL}{Paired-E}
\colorlet{vertex-LRRRLLLL}{Paired-B}
\colorlet{vertex-LLRLLRRL}{Paired-I}
\colorlet{vertex-RRLRLRLL}{Paired-I}
\colorlet{vertex-RRLRLRRL}{white}
\colorlet{vertex-RLLLRLRL}{Paired-D}
\colorlet{vertex-RLLRLLRL}{Paired-F}
\colorlet{vertex-RLLLLLRR}{Paired-D}
\colorlet{vertex-LLLRLLRR}{Paired-J}
\colorlet{vertex-LRLLRLLR}{Paired-F}
\colorlet{vertex-LRRRRLLL}{Paired-K}
\colorlet{vertex-LLRLRRLR}{white}
\colorlet{vertex-LLRLLRRR}{Paired-B}
\colorlet{vertex-RRLRLRRR}{Paired-G}
\colorlet{vertex-RLRRLRLR}{white}
\colorlet{vertex-LLLRRLLR}{Paired-A}
\colorlet{vertex-RLLRLRLL}{Paired-A}
\colorlet{vertex-LLRRLLLR}{Paired-K}
\colorlet{vertex-LRRRRRRR}{Paired-A}
\colorlet{vertex-LLLRLLLR}{Paired-D}
\colorlet{vertex-RLRLLLRR}{Paired-D}
\colorlet{vertex-LLRLRRLL}{Paired-J}
\colorlet{vertex-RLLLRLLR}{Paired-A}
\colorlet{vertex-LRRRRLRR}{Paired-C}
\colorlet{vertex-RLLRLLLL}{white}
\colorlet{vertex-LLLLRLRR}{white}
\colorlet{vertex-RLLLLLLLR}{Paired-G}
\colorlet{vertex-LRRRRRLLR}{Paired-G}
\colorlet{vertex-RRLRLRRRL}{Paired-A}
\colorlet{vertex-LRRRRLLLR}{Paired-F}
\colorlet{vertex-RLLRLRLRL}{Paired-I}
\colorlet{vertex-RRLRLRRRR}{Paired-F}
\colorlet{vertex-RLLRLRRRR}{Paired-K}
\colorlet{vertex-RLLRLRRLL}{Paired-I}
\colorlet{vertex-LRLLRLLRR}{Paired-K}
\colorlet{vertex-RLLLRLLRR}{white}
\colorlet{vertex-LLLLRRRRR}{Paired-K}
\colorlet{vertex-LLLRLLLRL}{Paired-C}
\colorlet{vertex-RLLRLLLRR}{Paired-J}
\colorlet{vertex-RLLLRLRRL}{Paired-H}
\colorlet{vertex-LLLRLLLRR}{Paired-H}
\colorlet{vertex-RLLLRLLLR}{Paired-C}
\colorlet{vertex-LRRRRLRRR}{Paired-B}
\colorlet{vertex-RLLRLLLRL}{Paired-D}
\colorlet{vertex-LLLLRRRLL}{Paired-F}
\colorlet{vertex-LRRRRLLRR}{Paired-G}
\colorlet{vertex-RLLLRLRRR}{Paired-K}
\colorlet{vertex-LRRRRLRLR}{Paired-G}
\colorlet{vertex-RLLRLRRLR}{Paired-B}
\colorlet{vertex-LRLLRRRLL}{Paired-I}
\colorlet{vertex-LRLLRRRRR}{Paired-E}
\colorlet{vertex-LLLRLRRLL}{Paired-H}
\colorlet{vertex-LLLRLLLLL}{Paired-E}
\colorlet{vertex-LLLLRRRRL}{Paired-D}
\colorlet{vertex-LLRRLLLRR}{Paired-I}
\colorlet{vertex-RLLLLLLRR}{Paired-C}
\colorlet{vertex-LLLRLRRLR}{white}
\colorlet{vertex-RRLRLRLRL}{Paired-J}
\colorlet{vertex-LRRRRLRLL}{Paired-F}
\colorlet{vertex-LRRRRLLRL}{Paired-E}
\colorlet{vertex-RLLLRLLLL}{Paired-J}
\colorlet{vertex-LLRLLRLRL}{Paired-H}
\colorlet{vertex-LRLLRLLRL}{Paired-G}
\colorlet{vertex-RLLLLLLRL}{Paired-J}
\colorlet{vertex-LRRRRRLLL}{Paired-K}
\colorlet{vertex-LLLRLLLLR}{Paired-A}
\colorlet{vertex-LRRRRLLLL}{Paired-D}
\colorlet{vertex-RLLRLRRRL}{Paired-H}
\colorlet{vertex-LLRRLLLRL}{Paired-G}
\colorlet{vertex-LRRRRLRRL}{Paired-H}
\colorlet{vertex-RLLRLLRRR}{Paired-E}
\colorlet{vertex-LRLLRRLLL}{white}
\colorlet{vertex-RLLLLLLLL}{Paired-I}
\colorlet{vertex-LRLLRRRLR}{Paired-D}
\colorlet{vertex-LLRLLRLRR}{Paired-A}
\colorlet{vertex-RLLLRLLRL}{Paired-D}
\colorlet{vertex-LRLLRRRRL}{Paired-C}
\colorlet{vertex-LLLLRRRLR}{Paired-C}
\colorlet{vertex-RLLRLRLRR}{Paired-H}
\colorlet{vertex-LRLLRRLLR}{Paired-F}
\colorlet{vertex-RRLRLRLRR}{Paired-G}
\colorlet{vertex-RLLRLLRRL}{Paired-G}
\colorlet{vertex-RLLRLRRLLR}{Paired-A}
\colorlet{vertex-RLLLRLLRLR}{Paired-H}
\colorlet{vertex-LRRRRLLRRL}{Paired-J}
\colorlet{vertex-LRRRRLLRLR}{Paired-C}
\colorlet{vertex-LRRRRLLLLL}{Paired-A}
\colorlet{vertex-LRLLRRRRRL}{Paired-D}
\colorlet{vertex-LLLLRRRRRR}{Paired-H}
\colorlet{vertex-LRRRRLLLLR}{Paired-E}
\colorlet{vertex-RLLRLLLRRR}{Paired-E}
\colorlet{vertex-RLLRLRLRRL}{Paired-B}
\colorlet{vertex-LRLLRRRRRR}{Paired-A}
\colorlet{vertex-LLLLRRRRRL}{Paired-C}
\colorlet{vertex-RLLLRLLLRL}{Paired-F}
\colorlet{vertex-RLLLRLLLRR}{Paired-K}
\colorlet{vertex-LRRRRLLLRR}{Paired-C}
\colorlet{vertex-RLLLRLLRLL}{Paired-F}
\colorlet{vertex-LRLLRRRLRR}{Paired-E}
\colorlet{vertex-LLLLRRRRLL}{Paired-E}
\colorlet{vertex-RLLRLRRLLL}{Paired-D}
\colorlet{vertex-LLLLRRRRLR}{Paired-H}
\colorlet{vertex-LRRRRLLLRL}{Paired-H}
\colorlet{vertex-LRLLRRRLRL}{Paired-J}
\colorlet{vertex-RLLRLRLRRR}{white}
\colorlet{vertex-LRRRRLLRLL}{Paired-D}
\colorlet{vertex-LRRRRLLRRR}{Paired-B}
\colorlet{vertex-RLLRLLLRRL}{Paired-C}
\colorlet{vertex-RLLLRLLLRRL}{white}
\colorlet{vertex-LLLLRRRRLRL}{Paired-F}
\colorlet{vertex-LRRRRLLLLLR}{Paired-H}
\colorlet{vertex-LRRRRLLLLLL}{Paired-K}
\colorlet{vertex-LLLLRRRRLRR}{Paired-A}
\colorlet{vertex-RLLLRLLLRRR}{Paired-G}
\colorlet{vertex-LRRRRLLLLLLR}{Paired-I}
\colorlet{vertex-LRRRRLLLLLLL}{Paired-D}
\colorlet{vertex-root}{Paired-K}
\colorlet{text-}{black}
\colorlet{text-L}{black}
\colorlet{text-R}{black}
\colorlet{text-RR}{white}
\colorlet{text-LR}{white}
\colorlet{text-LRL}{black}
\colorlet{text-LRR}{black}
\colorlet{text-LL}{white}
\colorlet{text-LRRL}{white}
\colorlet{text-LRRLL}{black}
\colorlet{text-LRRRR}{white}
\colorlet{text-RL}{black}
\colorlet{text-LLL}{black}
\colorlet{text-RLL}{black}
\colorlet{text-RRL}{black}
\colorlet{text-LLR}{white}
\colorlet{text-RLR}{white}
\colorlet{text-RRR}{black}
\colorlet{text-LRLR}{black}
\colorlet{text-RLLL}{black}
\colorlet{text-LLRR}{black}
\colorlet{text-RRLL}{black}
\colorlet{text-RRLR}{black}
\colorlet{text-RLRL}{black}
\colorlet{text-RRRR}{white}
\colorlet{text-LLLR}{black}
\colorlet{text-LLLL}{white}
\colorlet{text-LRLL}{black}
\colorlet{text-RLRR}{white}
\colorlet{text-LRRR}{white}
\colorlet{text-RRRL}{black}
\colorlet{text-LLRL}{black}
\colorlet{text-RLLR}{white}
\colorlet{text-LRRRL}{black}
\colorlet{text-LLLLR}{black}
\colorlet{text-RLLLL}{black}
\colorlet{text-RLRRL}{black}
\colorlet{text-RRRLR}{white}
\colorlet{text-RLLLR}{white}
\colorlet{text-LLRRR}{black}
\colorlet{text-RLRLR}{white}
\colorlet{text-RRRRR}{black}
\colorlet{text-RRLLL}{black}
\colorlet{text-RRLRL}{white}
\colorlet{text-LRLRL}{black}
\colorlet{text-RLRRR}{black}
\colorlet{text-RLLRR}{black}
\colorlet{text-RRRLL}{black}
\colorlet{text-LLLRL}{black}
\colorlet{text-LRRLR}{black}
\colorlet{text-RLRLL}{white}
\colorlet{text-LLRRL}{white}
\colorlet{text-LRLLR}{black}
\colorlet{text-RLLRL}{black}
\colorlet{text-LLLLL}{black}
\colorlet{text-LLRLL}{black}
\colorlet{text-LRLLL}{black}
\colorlet{text-LRLRR}{white}
\colorlet{text-LLLRR}{black}
\colorlet{text-RRRRL}{white}
\colorlet{text-RRLRR}{black}
\colorlet{text-LLRLR}{black}
\colorlet{text-RRLLR}{black}
\colorlet{text-LLRLLL}{white}
\colorlet{text-RRLRLR}{white}
\colorlet{text-RRLRRR}{black}
\colorlet{text-LRLRRR}{black}
\colorlet{text-LRLRLL}{white}
\colorlet{text-LRRRLR}{black}
\colorlet{text-LLRRRL}{black}
\colorlet{text-RLLLLR}{black}
\colorlet{text-LLRRRR}{white}
\colorlet{text-RRRLRL}{black}
\colorlet{text-RRRLLL}{white}
\colorlet{text-LRRRRL}{black}
\colorlet{text-LLLLLL}{black}
\colorlet{text-RLRLLR}{black}
\colorlet{text-LLLRLR}{black}
\colorlet{text-LRLRRL}{white}
\colorlet{text-RLLLRR}{black}
\colorlet{text-RLLLLL}{black}
\colorlet{text-RLLRLR}{white}
\colorlet{text-LLLLRR}{black}
\colorlet{text-RRRLLR}{black}
\colorlet{text-LLRLLR}{black}
\colorlet{text-LLRRLL}{white}
\colorlet{text-RLRLLL}{black}
\colorlet{text-LLLRLL}{white}
\colorlet{text-LLLRRR}{white}
\colorlet{text-RRLRRL}{white}
\colorlet{text-RRRLRR}{black}
\colorlet{text-RRLLLR}{black}
\colorlet{text-RLRRRR}{black}
\colorlet{text-RLRRLL}{black}
\colorlet{text-RLLRRL}{black}
\colorlet{text-LRLLLR}{black}
\colorlet{text-RRLLLL}{white}
\colorlet{text-LRLLLL}{white}
\colorlet{text-LLRLRL}{white}
\colorlet{text-LLRLRR}{black}
\colorlet{text-RRRRLR}{black}
\colorlet{text-LRRRRR}{white}
\colorlet{text-LLLRRL}{white}
\colorlet{text-RLRRLR}{black}
\colorlet{text-RRLLRR}{black}
\colorlet{text-LRRLLR}{black}
\colorlet{text-LRLRLR}{black}
\colorlet{text-LRLLRL}{white}
\colorlet{text-LRLLRR}{white}
\colorlet{text-LLLLLR}{black}
\colorlet{text-LRRRLL}{black}
\colorlet{text-RRLLRL}{white}
\colorlet{text-RRLRLL}{black}
\colorlet{text-LLRRLR}{black}
\colorlet{text-LRRLLL}{black}
\colorlet{text-LLLLRL}{white}
\colorlet{text-RLRRRL}{black}
\colorlet{text-RRRRLL}{black}
\colorlet{text-RLLLRL}{white}
\colorlet{text-RLLRRR}{black}
\colorlet{text-RLLRLL}{black}
\colorlet{text-LLRLRRR}{white}
\colorlet{text-RLLLLLR}{white}
\colorlet{text-LRRRLLR}{black}
\colorlet{text-LRRRLLL}{black}
\colorlet{text-RLRRLRR}{white}
\colorlet{text-RRLRRLR}{black}
\colorlet{text-LRLRRLR}{black}
\colorlet{text-RRLLLRR}{white}
\colorlet{text-RLRLLRL}{black}
\colorlet{text-LRLLLLR}{black}
\colorlet{text-LRRRRLL}{black}
\colorlet{text-RLLLLLL}{black}
\colorlet{text-LRLRRRR}{black}
\colorlet{text-RRLRLRL}{black}
\colorlet{text-LLRLLRL}{black}
\colorlet{text-LRLLLRR}{white}
\colorlet{text-LLLLLRL}{black}
\colorlet{text-LRRRLRR}{white}
\colorlet{text-LLLRRLR}{black}
\colorlet{text-LRLRLLR}{black}
\colorlet{text-LRRRLRL}{black}
\colorlet{text-LRLLRRR}{black}
\colorlet{text-LLRLLRR}{black}
\colorlet{text-RLRRLLR}{white}
\colorlet{text-LLRLLLR}{black}
\colorlet{text-RRLRLLR}{white}
\colorlet{text-LLRRRRL}{black}
\colorlet{text-LLLRLLR}{black}
\colorlet{text-LRLLLRL}{white}
\colorlet{text-RLRRLRL}{black}
\colorlet{text-LLLLRLL}{white}
\colorlet{text-RLLLRLR}{white}
\colorlet{text-RLLRLLL}{black}
\colorlet{text-LRRRRRR}{black}
\colorlet{text-LLLLRLR}{black}
\colorlet{text-LRLLRLL}{black}
\colorlet{text-LRLLRLR}{white}
\colorlet{text-LRLLRRL}{black}
\colorlet{text-RLRLLRR}{black}
\colorlet{text-RRLRLRR}{black}
\colorlet{text-LRLRLRR}{black}
\colorlet{text-LLRRRRR}{white}
\colorlet{text-LLLLRRL}{black}
\colorlet{text-LLLRLLL}{white}
\colorlet{text-LLLLRRR}{black}
\colorlet{text-RLRLLLR}{black}
\colorlet{text-LRLLLLL}{black}
\colorlet{text-LRLRLRL}{black}
\colorlet{text-RRLRRLL}{black}
\colorlet{text-LRRRRRL}{white}
\colorlet{text-RRLLLRL}{white}
\colorlet{text-RLRRRRL}{black}
\colorlet{text-LLLRRRR}{black}
\colorlet{text-RLLLRLL}{black}
\colorlet{text-LLRLRRL}{black}
\colorlet{text-RLRRLLL}{black}
\colorlet{text-LLRLLLL}{white}
\colorlet{text-LLLLLRR}{black}
\colorlet{text-LLLRRRL}{black}
\colorlet{text-RLLRLRR}{black}
\colorlet{text-LRLRRLL}{black}
\colorlet{text-RLRLLLL}{white}
\colorlet{text-LRRRRLR}{black}
\colorlet{text-LLRRLLL}{black}
\colorlet{text-RLLRLLR}{white}
\colorlet{text-LLLRLRR}{white}
\colorlet{text-LRLRLLL}{white}
\colorlet{text-LLLRLRL}{black}
\colorlet{text-RLLRLRL}{black}
\colorlet{text-RLRRRRR}{white}
\colorlet{text-LRLRRRL}{black}
\colorlet{text-LLRRLLR}{black}
\colorlet{text-LLLRRLL}{white}
\colorlet{text-RRLRLLL}{white}
\colorlet{text-RLLLLLLR}{black}
\colorlet{text-LRRRLLLR}{white}
\colorlet{text-LLLLRRRL}{black}
\colorlet{text-LRRRRRLL}{black}
\colorlet{text-RRLRLLLR}{black}
\colorlet{text-LLLRLLLL}{black}
\colorlet{text-LLLRLLRL}{black}
\colorlet{text-RRLRLLLL}{white}
\colorlet{text-LRRRRLLR}{black}
\colorlet{text-LRLLRRLL}{black}
\colorlet{text-LLLRLRLR}{black}
\colorlet{text-LRLLRRRL}{black}
\colorlet{text-LRLLRRLR}{white}
\colorlet{text-RLLRLRRL}{white}
\colorlet{text-RLLLRLRR}{black}
\colorlet{text-RRLRRLLL}{white}
\colorlet{text-LRRRRRRL}{black}
\colorlet{text-RLRRLLLL}{white}
\colorlet{text-RLLLLLRL}{white}
\colorlet{text-LLLLRLRL}{black}
\colorlet{text-RRLRRLLR}{black}
\colorlet{text-RLRLLLLL}{black}
\colorlet{text-RRLRLRLR}{black}
\colorlet{text-LLRLLRLL}{white}
\colorlet{text-LLLLRRRR}{white}
\colorlet{text-LLLLRLLR}{black}
\colorlet{text-LLLRLRLL}{white}
\colorlet{text-LRLRRLLL}{white}
\colorlet{text-LLRLLRLR}{white}
\colorlet{text-LRLRLRLL}{white}
\colorlet{text-RLRRLRLL}{black}
\colorlet{text-LLLRRRLR}{black}
\colorlet{text-RLLRLRRR}{black}
\colorlet{text-RLRRLLLR}{black}
\colorlet{text-RLRLLLLR}{white}
\colorlet{text-RLLRLLLR}{black}
\colorlet{text-LRLRRLLR}{white}
\colorlet{text-RLLRLLRR}{black}
\colorlet{text-RLLRLRLR}{black}
\colorlet{text-LRRRRRLR}{black}
\colorlet{text-LLLRLRRR}{black}
\colorlet{text-RLLLLLLL}{black}
\colorlet{text-LRLLRLLL}{black}
\colorlet{text-LLLRRLLL}{white}
\colorlet{text-LLLRRRLL}{black}
\colorlet{text-LRLRLRLR}{black}
\colorlet{text-LRRRRLRL}{black}
\colorlet{text-LRLLRRRR}{black}
\colorlet{text-RLRLLLRL}{black}
\colorlet{text-LLLRLRRL}{white}
\colorlet{text-RLLLRLLL}{black}
\colorlet{text-LLLLRLLL}{white}
\colorlet{text-LLRRLLLL}{black}
\colorlet{text-LRRRLLLL}{white}
\colorlet{text-LLRLLRRL}{black}
\colorlet{text-RRLRLRLL}{black}
\colorlet{text-RRLRLRRL}{black}
\colorlet{text-RLLLRLRL}{white}
\colorlet{text-RLLRLLRL}{white}
\colorlet{text-RLLLLLRR}{white}
\colorlet{text-LLLRLLRR}{white}
\colorlet{text-LRLLRLLR}{white}
\colorlet{text-LRRRRLLL}{black}
\colorlet{text-LLRLRRLR}{black}
\colorlet{text-LLRLLRRR}{white}
\colorlet{text-RRLRLRRR}{black}
\colorlet{text-RLRRLRLR}{black}
\colorlet{text-LLLRRLLR}{black}
\colorlet{text-RLLRLRLL}{black}
\colorlet{text-LLRRLLLR}{black}
\colorlet{text-LRRRRRRR}{black}
\colorlet{text-LLLRLLLR}{white}
\colorlet{text-RLRLLLRR}{white}
\colorlet{text-LLRLRRLL}{white}
\colorlet{text-RLLLRLLR}{black}
\colorlet{text-LRRRRLRR}{black}
\colorlet{text-RLLRLLLL}{black}
\colorlet{text-LLLLRLRR}{black}
\colorlet{text-RLLLLLLLR}{black}
\colorlet{text-LRRRRRLLR}{black}
\colorlet{text-RRLRLRRRL}{black}
\colorlet{text-LRRRRLLLR}{white}
\colorlet{text-RLLRLRLRL}{black}
\colorlet{text-RRLRLRRRR}{white}
\colorlet{text-RLLRLRRRR}{black}
\colorlet{text-RLLRLRRLL}{black}
\colorlet{text-LRLLRLLRR}{black}
\colorlet{text-RLLLRLLRR}{black}
\colorlet{text-LLLLRRRRR}{black}
\colorlet{text-LLLRLLLRL}{black}
\colorlet{text-RLLRLLLRR}{white}
\colorlet{text-RLLLRLRRL}{black}
\colorlet{text-LLLRLLLRR}{black}
\colorlet{text-RLLLRLLLR}{black}
\colorlet{text-LRRRRLRRR}{white}
\colorlet{text-RLLRLLLRL}{white}
\colorlet{text-LLLLRRRLL}{white}
\colorlet{text-LRRRRLLRR}{black}
\colorlet{text-RLLLRLRRR}{black}
\colorlet{text-LRRRRLRLR}{black}
\colorlet{text-RLLRLRRLR}{white}
\colorlet{text-LRLLRRRLL}{black}
\colorlet{text-LRLLRRRRR}{black}
\colorlet{text-LLLRLRRLL}{black}
\colorlet{text-LLLRLLLLL}{black}
\colorlet{text-LLLLRRRRL}{white}
\colorlet{text-LLRRLLLRR}{black}
\colorlet{text-RLLLLLLRR}{black}
\colorlet{text-LLLRLRRLR}{black}
\colorlet{text-RRLRLRLRL}{white}
\colorlet{text-LRRRRLRLL}{white}
\colorlet{text-LRRRRLLRL}{black}
\colorlet{text-RLLLRLLLL}{white}
\colorlet{text-LLRLLRLRL}{black}
\colorlet{text-LRLLRLLRL}{black}
\colorlet{text-RLLLLLLRL}{white}
\colorlet{text-LRRRRRLLL}{black}
\colorlet{text-LLLRLLLLR}{black}
\colorlet{text-LRRRRLLLL}{white}
\colorlet{text-RLLRLRRRL}{black}
\colorlet{text-LLRRLLLRL}{black}
\colorlet{text-LRRRRLRRL}{black}
\colorlet{text-RLLRLLRRR}{black}
\colorlet{text-LRLLRRLLL}{black}
\colorlet{text-RLLLLLLLL}{black}
\colorlet{text-LRLLRRRLR}{white}
\colorlet{text-LLRLLRLRR}{black}
\colorlet{text-RLLLRLLRL}{white}
\colorlet{text-LRLLRRRRL}{black}
\colorlet{text-LLLLRRRLR}{black}
\colorlet{text-RLLRLRLRR}{black}
\colorlet{text-LRLLRRLLR}{white}
\colorlet{text-RRLRLRLRR}{black}
\colorlet{text-RLLRLLRRL}{black}
\colorlet{text-RLLRLRRLLR}{black}
\colorlet{text-RLLLRLLRLR}{black}
\colorlet{text-LRRRRLLRRL}{white}
\colorlet{text-LRRRRLLRLR}{black}
\colorlet{text-LRRRRLLLLL}{black}
\colorlet{text-LRLLRRRRRL}{white}
\colorlet{text-LLLLRRRRRR}{black}
\colorlet{text-LRRRRLLLLR}{black}
\colorlet{text-RLLRLLLRRR}{black}
\colorlet{text-RLLRLRLRRL}{white}
\colorlet{text-LRLLRRRRRR}{black}
\colorlet{text-LLLLRRRRRL}{black}
\colorlet{text-RLLLRLLLRL}{white}
\colorlet{text-RLLLRLLLRR}{black}
\colorlet{text-LRRRRLLLRR}{black}
\colorlet{text-RLLLRLLRLL}{white}
\colorlet{text-LRLLRRRLRR}{black}
\colorlet{text-LLLLRRRRLL}{black}
\colorlet{text-RLLRLRRLLL}{white}
\colorlet{text-LLLLRRRRLR}{black}
\colorlet{text-LRRRRLLLRL}{black}
\colorlet{text-LRLLRRRLRL}{white}
\colorlet{text-RLLRLRLRRR}{black}
\colorlet{text-LRRRRLLRLL}{white}
\colorlet{text-LRRRRLLRRR}{white}
\colorlet{text-RLLRLLLRRL}{black}
\colorlet{text-RLLLRLLLRRL}{black}
\colorlet{text-LLLLRRRRLRL}{white}
\colorlet{text-LRRRRLLLLLR}{black}
\colorlet{text-LRRRRLLLLLL}{black}
\colorlet{text-LLLLRRRRLRR}{black}
\colorlet{text-RLLLRLLLRRR}{black}
\colorlet{text-LRRRRLLLLLLR}{black}
\colorlet{text-LRRRRLLLLLLL}{white}
\colorlet{text-root}{black}


==> figures/autogenerated/_jdt-slide-color-scheme.tex <==
% AUTO-GENERATED z-index color scheme for the jeu-de-taquin-slide figures.
% Source: notebooks/figures/08_jdt_slide_figures.ipynb in trees-SageMath
% (orchestrated by SageMath/libraries/visualization/jdt_slide.py).
% To regenerate, run that notebook; do not edit by hand.
\colorlet{vertex-z1}{Paired-K}%
\colorlet{vertex-z2}{Paired-A}%
\colorlet{vertex-z3}{Paired-H}%
\colorlet{vertex-z4}{Paired-H}%
\colorlet{vertex-z5}{Paired-I}%
\colorlet{vertex-z6}{white}%
\colorlet{vertex-z7}{Paired-K}%
\colorlet{vertex-z8}{Paired-J}%
\colorlet{vertex-z9}{Paired-G}%
\colorlet{vertex-z10}{Paired-G}%
\colorlet{vertex-z11}{Paired-E}%
\colorlet{vertex-z12}{Paired-C}%
\colorlet{vertex-z13}{Paired-F}%
\colorlet{vertex-z14}{Paired-C}%
\colorlet{vertex-z15}{Paired-J}%
\colorlet{vertex-z16}{Paired-E}%
\colorlet{vertex-z19}{Paired-A}%
\colorlet{vertex-z20}{Paired-B}%
\colorlet{vertex-z21}{white}%
\colorlet{vertex-z22}{Paired-C}%
\colorlet{vertex-z23}{Paired-J}%
\colorlet{vertex-z24}{white}%
\colorlet{vertex-z27}{Paired-F}%
\colorlet{vertex-z31}{Paired-F}%
\colorlet{vertex-z32}{Paired-H}%
\colorlet{vertex-z33}{Paired-F}%
\colorlet{vertex-z34}{Paired-E}%
\colorlet{vertex-z35}{Paired-B}%
\colorlet{vertex-z37}{Paired-J}%
\colorlet{vertex-z39}{Paired-D}%
\colorlet{vertex-z40}{Paired-L}%
\colorlet{vertex-z42}{Paired-G}%
\colorlet{vertex-z44}{Paired-E}%
\colorlet{vertex-z46}{Paired-B}%
\colorlet{vertex-z48}{Paired-B}%
\colorlet{vertex-z51}{Paired-I}%
\colorlet{vertex-z54}{Paired-C}%
\colorlet{vertex-z56}{Paired-I}%
\colorlet{vertex-z59}{Paired-B}%
\colorlet{vertex-z60}{Paired-E}%
\colorlet{vertex-z62}{Paired-D}%
\colorlet{vertex-z63}{Paired-H}%
\colorlet{vertex-z66}{white}%
\colorlet{vertex-z72}{Paired-A}%
\colorlet{vertex-z73}{Paired-J}%
\colorlet{vertex-z74}{Paired-K}%
\colorlet{vertex-z80}{Paired-A}%
\colorlet{vertex-z84}{white}%
\colorlet{vertex-z87}{Paired-J}%
\colorlet{vertex-z89}{Paired-H}%
\colorlet{vertex-z90}{Paired-D}%
\colorlet{vertex-z102}{Paired-C}%
\colorlet{vertex-z122}{Paired-F}%
\colorlet{vertex-z141}{Paired-D}%
\colorlet{vertex-z150}{Paired-A}%
\colorlet{vertex-z180}{Paired-K}%
\colorlet{vertex-z203}{Paired-G}%
\colorlet{vertex-z220}{Paired-C}%
\colorlet{vertex-z277}{Paired-H}%
\colorlet{vertex-z347}{Paired-G}%
\colorlet{vertex-z359}{Paired-F}%
\colorlet{vertex-z398}{Paired-D}%
\colorlet{vertex-z492}{Paired-J}%


==> figures/autogenerated/binary-tree-color-scheme.tex <==
% Generated by 02_generate_color_scheme.ipynb
% Date: 2025-10-31 08:25:09.999282

\colorlet{vertex-}{Paired-K}
\colorlet{vertex-L}{Paired-A}
\colorlet{vertex-R}{Paired-H}
\colorlet{vertex-RR}{Paired-J}
\colorlet{vertex-LR}{Paired-F}
\colorlet{vertex-LRL}{white}
\colorlet{vertex-LRR}{Paired-C}
\colorlet{vertex-LL}{Paired-K}
\colorlet{vertex-LRRL}{Paired-J}
\colorlet{vertex-LRRLL}{Paired-L}
\colorlet{vertex-LRRRR}{Paired-D}
\colorlet{vertex-RL}{Paired-I}
\colorlet{vertex-LLL}{Paired-G}
\colorlet{vertex-LLR}{Paired-E}
\colorlet{vertex-RLL}{Paired-B}
\colorlet{vertex-RLR}{Paired-G}
\colorlet{vertex-RRL}{Paired-E}
\colorlet{vertex-RRR}{white}
\colorlet{vertex-LLLL}{Paired-D}
\colorlet{vertex-LLLR}{Paired-B}
\colorlet{vertex-LLRL}{Paired-I}
\colorlet{vertex-LLRR}{Paired-D}
\colorlet{vertex-LRLL}{Paired-H}
\colorlet{vertex-LRLR}{Paired-G}
\colorlet{vertex-LRRR}{Paired-E}
\colorlet{vertex-RLLL}{Paired-G}
\colorlet{vertex-RLLR}{white}
\colorlet{vertex-RLRL}{Paired-E}
\colorlet{vertex-RLRR}{Paired-D}
\colorlet{vertex-RRLL}{white}
\colorlet{vertex-RRLR}{Paired-B}
\colorlet{vertex-RRRL}{Paired-C}
\colorlet{vertex-RRRR}{Paired-F}
\colorlet{vertex-LLLLL}{Paired-J}
\colorlet{vertex-LLLLR}{Paired-C}
\colorlet{vertex-LLLRL}{Paired-H}
\colorlet{vertex-LLLRR}{Paired-J}
\colorlet{vertex-LLRLL}{white}
\colorlet{vertex-LLRLR}{Paired-C}
\colorlet{vertex-LRLLL}{Paired-C}
\colorlet{vertex-LRLLR}{Paired-B}
\colorlet{vertex-LRLRL}{Paired-I}
\colorlet{vertex-LRLRR}{Paired-D}
\colorlet{vertex-LRRLR}{Paired-G}
\colorlet{vertex-LRRRL}{Paired-B}
\colorlet{vertex-RLLRL}{Paired-J}
\colorlet{vertex-RLLRR}{Paired-C}
\colorlet{vertex-RLRLL}{Paired-J}
\colorlet{vertex-RLRLR}{Paired-F}
\colorlet{vertex-RLRRL}{Paired-A}
\colorlet{vertex-RLRRR}{Paired-K}
\colorlet{vertex-RRLLL}{Paired-B}
\colorlet{vertex-RRLLR}{Paired-F}
\colorlet{vertex-RRRLL}{Paired-A}
\colorlet{vertex-RRRLR}{Paired-D}
\colorlet{vertex-RRRRL}{Paired-G}
\colorlet{vertex-RRRRR}{Paired-I}
\colorlet{vertex-LLLLLL}{Paired-F}
\colorlet{vertex-LLLLLR}{white}
\colorlet{vertex-LLLRLL}{Paired-F}
\colorlet{vertex-LLLRLR}{white}
\colorlet{vertex-LLLRRL}{Paired-F}
\colorlet{vertex-LLLRRR}{Paired-C}
\colorlet{vertex-LLRLLL}{Paired-A}
\colorlet{vertex-LLRLLR}{Paired-H}
\colorlet{vertex-LLRLRL}{Paired-F}
\colorlet{vertex-LLRLRR}{Paired-B}
\colorlet{vertex-LRLLLL}{Paired-F}
\colorlet{vertex-LRLLLR}{Paired-J}
\colorlet{vertex-LRLRLL}{Paired-J}
\colorlet{vertex-LRLRLR}{Paired-E}
\colorlet{vertex-LRLRRL}{Paired-B}
\colorlet{vertex-LRLRRR}{Paired-A}
\colorlet{vertex-LRRLLL}{Paired-I}
\colorlet{vertex-LRRLLR}{Paired-H}
\colorlet{vertex-LRRRLL}{Paired-I}
\colorlet{vertex-LRRRLR}{white}
\colorlet{vertex-LRRRRL}{Paired-A}
\colorlet{vertex-LRRRRR}{Paired-F}
\colorlet{vertex-RLLRRL}{Paired-D}
\colorlet{vertex-RLLRRR}{Paired-K}
\colorlet{vertex-RLRLLL}{Paired-H}
\colorlet{vertex-RLRLLR}{Paired-A}
\colorlet{vertex-RLRRLL}{Paired-J}
\colorlet{vertex-RLRRLR}{Paired-C}
\colorlet{vertex-RRRLLL}{Paired-F}
\colorlet{vertex-RRRLLR}{Paired-I}
\colorlet{vertex-RRRRLL}{Paired-K}
\colorlet{vertex-RRRRLR}{Paired-A}
\colorlet{vertex-LLLRRLL}{Paired-I}
\colorlet{vertex-LLLRRLR}{Paired-D}
\colorlet{vertex-LLRLLLL}{Paired-E}
\colorlet{vertex-LLRLLLR}{Paired-D}
\colorlet{vertex-LLRLLRL}{Paired-F}
\colorlet{vertex-LLRLLRR}{Paired-J}
\colorlet{vertex-LLRLRRL}{Paired-G}
\colorlet{vertex-LLRLRRR}{Paired-J}
\colorlet{vertex-LRLLLLL}{white}
\colorlet{vertex-LRLLLLR}{Paired-I}
\colorlet{vertex-LRLRLLL}{Paired-F}
\colorlet{vertex-LRLRLLR}{Paired-C}
\colorlet{vertex-LRLRLRL}{Paired-K}
\colorlet{vertex-LRLRLRR}{Paired-H}
\colorlet{vertex-LRLRRLL}{Paired-K}
\colorlet{vertex-LRLRRLR}{Paired-H}
\colorlet{vertex-LRRRRLL}{Paired-H}
\colorlet{vertex-LRRRRLR}{Paired-J}
\colorlet{vertex-LRRRRRL}{white}
\colorlet{vertex-LRRRRRR}{Paired-C}
\colorlet{vertex-RLRLLLL}{Paired-G}
\colorlet{vertex-RLRLLLR}{Paired-D}
\colorlet{vertex-LLRLLRLL}{Paired-E}
\colorlet{vertex-LLRLLRLR}{Paired-B}
\colorlet{vertex-LLRLLRRL}{Paired-G}
\colorlet{vertex-LLRLLRRR}{Paired-K}
\colorlet{vertex-LLRLRRLL}{Paired-D}
\colorlet{vertex-LLRLRRLR}{Paired-H}
\colorlet{vertex-LRLRLRLL}{Paired-D}
\colorlet{vertex-LRLRLRLR}{Paired-A}
\colorlet{vertex-LRLRRLLL}{Paired-F}
\colorlet{vertex-LRLRRLLR}{Paired-J}
\colorlet{vertex-LRRRRLLL}{Paired-K}
\colorlet{vertex-LRRRRLLR}{Paired-G}
\colorlet{vertex-RLRLLLRL}{Paired-F}
\colorlet{vertex-RLRLLLRR}{Paired-C}
\colorlet{vertex-root}{Paired-K}
\colorlet{text-}{black}
\colorlet{text-L}{black}
\colorlet{text-R}{black}
\colorlet{text-RR}{white}
\colorlet{text-LR}{white}
\colorlet{text-LRL}{black}
\colorlet{text-LRR}{black}
\colorlet{text-LL}{black}
\colorlet{text-LRRL}{white}
\colorlet{text-LRRLL}{black}
\colorlet{text-LRRRR}{white}
\colorlet{text-RL}{black}
\colorlet{text-LLL}{black}
\colorlet{text-LLR}{black}
\colorlet{text-RLL}{white}
\colorlet{text-RLR}{black}
\colorlet{text-RRL}{black}
\colorlet{text-RRR}{black}
\colorlet{text-LLLL}{white}
\colorlet{text-LLLR}{white}
\colorlet{text-LLRL}{black}
\colorlet{text-LLRR}{white}
\colorlet{text-LRLL}{black}
\colorlet{text-LRLR}{black}
\colorlet{text-LRRR}{black}
\colorlet{text-RLLL}{black}
\colorlet{text-RLLR}{black}
\colorlet{text-RLRL}{black}
\colorlet{text-RLRR}{white}
\colorlet{text-RRLL}{black}
\colorlet{text-RRLR}{white}
\colorlet{text-RRRL}{black}
\colorlet{text-RRRR}{white}
\colorlet{text-LLLLL}{white}
\colorlet{text-LLLLR}{black}
\colorlet{text-LLLRL}{black}
\colorlet{text-LLLRR}{white}
\colorlet{text-LLRLL}{black}
\colorlet{text-LLRLR}{black}
\colorlet{text-LRLLL}{black}
\colorlet{text-LRLLR}{white}
\colorlet{text-LRLRL}{black}
\colorlet{text-LRLRR}{white}
\colorlet{text-LRRLR}{black}
\colorlet{text-LRRRL}{white}
\colorlet{text-RLLRL}{white}
\colorlet{text-RLLRR}{black}
\colorlet{text-RLRLL}{white}
\colorlet{text-RLRLR}{white}
\colorlet{text-RLRRL}{black}
\colorlet{text-RLRRR}{black}
\colorlet{text-RRLLL}{white}
\colorlet{text-RRLLR}{white}
\colorlet{text-RRRLL}{black}
\colorlet{text-RRRLR}{white}
\colorlet{text-RRRRL}{black}
\colorlet{text-RRRRR}{black}
\colorlet{text-LLLLLL}{white}
\colorlet{text-LLLLLR}{black}
\colorlet{text-LLLRLL}{white}
\colorlet{text-LLLRLR}{black}
\colorlet{text-LLLRRL}{white}
\colorlet{text-LLLRRR}{black}
\colorlet{text-LLRLLL}{black}
\colorlet{text-LLRLLR}{black}
\colorlet{text-LLRLRL}{white}
\colorlet{text-LLRLRR}{white}
\colorlet{text-LRLLLL}{white}
\colorlet{text-LRLLLR}{white}
\colorlet{text-LRLRLL}{white}
\colorlet{text-LRLRLR}{black}
\colorlet{text-LRLRRL}{white}
\colorlet{text-LRLRRR}{black}
\colorlet{text-LRRLLL}{black}
\colorlet{text-LRRLLR}{black}
\colorlet{text-LRRRLL}{black}
\colorlet{text-LRRRLR}{black}
\colorlet{text-LRRRRL}{black}
\colorlet{text-LRRRRR}{white}
\colorlet{text-RLLRRL}{white}
\colorlet{text-RLLRRR}{black}
\colorlet{text-RLRLLL}{black}
\colorlet{text-RLRLLR}{black}
\colorlet{text-RLRRLL}{white}
\colorlet{text-RLRRLR}{black}
\colorlet{text-RRRLLL}{white}
\colorlet{text-RRRLLR}{black}
\colorlet{text-RRRRLL}{black}
\colorlet{text-RRRRLR}{black}
\colorlet{text-LLLRRLL}{black}
\colorlet{text-LLLRRLR}{white}
\colorlet{text-LLRLLLL}{black}
\colorlet{text-LLRLLLR}{white}
\colorlet{text-LLRLLRL}{white}
\colorlet{text-LLRLLRR}{white}
\colorlet{text-LLRLRRL}{black}
\colorlet{text-LLRLRRR}{white}
\colorlet{text-LRLLLLL}{black}
\colorlet{text-LRLLLLR}{black}
\colorlet{text-LRLRLLL}{white}
\colorlet{text-LRLRLLR}{black}
\colorlet{text-LRLRLRL}{black}
\colorlet{text-LRLRLRR}{black}
\colorlet{text-LRLRRLL}{black}
\colorlet{text-LRLRRLR}{black}
\colorlet{text-LRRRRLL}{black}
\colorlet{text-LRRRRLR}{white}
\colorlet{text-LRRRRRL}{black}
\colorlet{text-LRRRRRR}{black}
\colorlet{text-RLRLLLL}{black}
\colorlet{text-RLRLLLR}{white}
\colorlet{text-LLRLLRLL}{black}
\colorlet{text-LLRLLRLR}{white}
\colorlet{text-LLRLLRRL}{black}
\colorlet{text-LLRLLRRR}{black}
\colorlet{text-LLRLRRLL}{white}
\colorlet{text-LLRLRRLR}{black}
\colorlet{text-LRLRLRLL}{white}
\colorlet{text-LRLRLRLR}{black}
\colorlet{text-LRLRRLLL}{white}
\colorlet{text-LRLRRLLR}{white}
\colorlet{text-LRRRRLLL}{black}
\colorlet{text-LRRRRLLR}{black}
\colorlet{text-RLRLLLRL}{white}
\colorlet{text-RLRLLLRR}{black}
\colorlet{text-root}{black}


==> figures/autogenerated/binary-tree-competition-content.tex <==
% Generated by 06_binary_tree_figure.ipynb

% Abstract binary tree with t^(1/4) time scaling; vertical axis: raw direction z in [0,1]

\node[node_style, fill=vertex-RRRRR, text=text-RRRRR] (node115) at (30,0.00022486378558778108) {};
\node[node_style, fill=vertex-RRRRLR, text=text-RRRRLR] (node114) at (30,0.001548097567753981) {};
\node[node_style, fill=vertex-RRRRLL, text=text-RRRRLL] (node113) at (30,0.0035909766246167707) {};
\node[node_style, fill=vertex-RRRRL, text=text-RRRRL] (node112) at (28.5137372095245,0.0026464675643324) {$z_{347}$};
\node[node_style, fill=vertex-RRRR, text=text-RRRR] (node111) at (23.9186045092711,0.00044972757117556217) {$z_{359}$};
\node[node_style, fill=vertex-RRRLR, text=text-RRRLR] (node110) at (30,0.011974607601945297) {};
\node[node_style, fill=vertex-RRRLL, text=text-RRRLL] (node109) at (30,0.029866587596993344) {$z_{80}$};
\node[node_style, fill=vertex-RRRL, text=text-RRRL] (node108) at (22.1747476241976,0.019413729518989453) {$z_{220}$};
\node[node_style, fill=vertex-RRR, text=text-RRR] (node107) at (12.9604479918725,0.004535485684901142) {$z_{84}$};
\node[node_style, fill=vertex-RRLR, text=text-RRLR] (node106) at (30,0.039366183650915265) {};
\node[node_style, fill=vertex-RRLLR, text=text-RRLLR] (node105) at (30,0.05091535456330548) {};
\node[node_style, fill=vertex-RRLLL, text=text-RRLLL] (node104) at (30,0.06110268728561896) {};
\node[node_style, fill=vertex-RRLL, text=text-RRLL] (node103) at (21.2669224779276,0.05737086893597898) {$z_{6}$};
\node[node_style, fill=vertex-RRL, text=text-RRL] (node102) at (11.6889216622419,0.04445984019063198) {$z_{60}$};
\node[node_style, fill=vertex-RR, text=text-RR] (node101) at (4.03089032463945,0.03427252711119855) {$z_{37}$};
\node[node_style, fill=vertex-RLRRR, text=text-RLRRR] (node100) at (30,0.07125189928718006) {};
\node[node_style, fill=vertex-RLRRLR, text=text-RLRRLR] (node99) at (30,0.08694615669749023) {};
\node[node_style, fill=vertex-RLRRLL, text=text-RLRRLL] (node98) at (30,0.10278851462894428) {};
\node[node_style, fill=vertex-RLRRL, text=text-RLRRL] (node97) at (28.7875932919399,0.09622302045587927) {$z_{150}$};
\node[node_style, fill=vertex-RLRR, text=text-RLRR] (node96) at (18.7139731873337,0.07766929293910119) {$z_{90}$};
\node[node_style, fill=vertex-RLRLR, text=text-RLRLR] (node95) at (30,0.11292366317848312) {};
\node[node_style, fill=vertex-RLRLLR, text=text-RLRLLR] (node94) at (30,0.12223229158302878) {};
\node[node_style, fill=vertex-RLRLLLR, text=text-RLRLLLR] (node93) at (30,0.13952285105739015) {$z_{141}$};
\node[node_style, fill=vertex-RLRLLLL, text=text-RLRLLLL] (node92) at (30,0.16399246909241827) {};
\node[node_style, fill=vertex-RLRLLL, text=text-RLRLLL] (node91) at (29.4960741558978,0.15359973329570875) {$z_{32}$};
\node[node_style, fill=vertex-RLRLL, text=text-RLRLL] (node90) at (21.5792751435628,0.12797126561110062) {$z_{8}$};
\node[node_style, fill=vertex-RLRL, text=text-RLRL] (node89) at (17.8149381545704,0.11649331755495695) {$z_{11}$};
\node[node_style, fill=vertex-RLR, text=text-RLR] (node88) at (12.6890670216942,0.1093540088020093) {$z_{10}$};
\node[node_style, fill=vertex-RLLRR, text=text-RLLRR] (node87) at (30,0.17894992229234052) {$z_{12}$};
\node[node_style, fill=vertex-RLLRL, text=text-RLLRL] (node86) at (30,0.20811766328654557) {};
\node[node_style, fill=vertex-RLLR, text=text-RLLR] (node85) at (20.9889233200760,0.20565181894893747) {$z_{66}$};
\node[node_style, fill=vertex-RLLL, text=text-RLLL] (node84) at (30,0.2152924121423938) {};
\node[node_style, fill=vertex-RLL, text=text-RLL] (node83) at (20.4330438587588,0.21058350762415368) {$z_{46}$};
\node[node_style, fill=vertex-RL, text=text-RL] (node82) at (6.17612032310910,0.1743852048891278) {$z_{5}$};
\node[node_style, fill=vertex-R, text=text-R] (node81) at (1.89882892211594,0.06483450563525894) {$z_{3}$};
\node[node_style, fill=vertex-LRRRRRR, text=text-LRRRRRR] (node80) at (30,0.2284977053015117) {};
\node[node_style, fill=vertex-LRRRRRL, text=text-LRRRRRL] (node79) at (30,0.2516502199303202) {};
\node[node_style, fill=vertex-LRRRRR, text=text-LRRRRR] (node78) at (24.5555349085051,0.23699409394238946) {$z_{31}$};
\node[node_style, fill=vertex-LRRRRLR, text=text-LRRRRLR] (node77) at (30,0.2861517023091808) {};
\node[node_style, fill=vertex-LRRRRLLR, text=text-LRRRRLLR] (node76) at (30,0.3139762790431894) {};
\node[node_style, fill=vertex-LRRRRLLL, text=text-LRRRRLLL] (node75) at (30,0.3313744294200838) {};
\node[node_style, fill=vertex-LRRRRLL, text=text-LRRRRLL] (node74) at (23.0782957685424,0.3219554993862682) {$z_{89}$};
\node[node_style, fill=vertex-LRRRRL, text=text-LRRRRL] (node73) at (15.0173771874149,0.3059970587001106) {$z_{72}$};
\node[node_style, fill=vertex-LRRRR, text=text-LRRRR] (node72) at (10.7771266702158,0.266306345918251) {$z_{39}$};
\node[node_style, fill=vertex-LRRRLR, text=text-LRRRLR] (node71) at (30,0.35248313830128813) {};
\node[node_style, fill=vertex-LRRRLL, text=text-LRRRLL] (node70) at (30,0.38385440149018907) {};
\node[node_style, fill=vertex-LRRRL, text=text-LRRRL] (node69) at (10.6268142614949,0.36417291714867683) {$z_{20}$};
\node[node_style, fill=vertex-LRRR, text=text-LRRR] (node68) at (6.61000034416844,0.34079335945389944) {$z_{16}$};
\node[node_style, fill=vertex-LRRLR, text=text-LRRLR] (node67) at (30,0.41168192952330807) {};
\node[node_style, fill=vertex-LRRLLR, text=text-LRRLLR] (node66) at (30,0.434981880632417) {};
\node[node_style, fill=vertex-LRRLLL, text=text-LRRLLL] (node65) at (30,0.4537423407531062) {};
\node[node_style, fill=vertex-LRRLL, text=text-LRRLL] (node64) at (18.8819410756336,0.45013578804991916) {$z_{40}$};
\node[node_style, fill=vertex-LRRL, text=text-LRRL] (node63) at (10.3858392624392,0.41982797321491483) {$z_{15}$};
\node[node_style, fill=vertex-LRR, text=text-LRR] (node62) at (3.39596269041207,0.4035358858317013) {$z_{14}$};
\node[node_style, fill=vertex-LRLRRR, text=text-LRLRRR] (node61) at (30,0.4841143318667406) {};
\node[node_style, fill=vertex-LRLRRLR, text=text-LRLRRLR] (node60) at (30,0.5137234829266881) {};
\node[node_style, fill=vertex-LRLRRLLR, text=text-LRLRRLLR] (node59) at (30,0.523679391635476) {};
\node[node_style, fill=vertex-LRLRRLLL, text=text-LRLRRLLL] (node58) at (30,0.5401467172962766) {};
\node[node_style, fill=vertex-LRLRRLL, text=text-LRLRRLL] (node57) at (29.5746308618543,0.5307915876947638) {$z_{180}$};
\node[node_style, fill=vertex-LRLRRL, text=text-LRLRRL] (node56) at (23.7802020724505,0.5165671955761885) {$z_{59}$};
\node[node_style, fill=vertex-LRLRR, text=text-LRLRR] (node55) at (22.2871763573938,0.5108797702771879) {$z_{62}$};
\node[node_style, fill=vertex-LRLRLRR, text=text-LRLRLRR] (node54) at (30,0.5534374361305631) {};
\node[node_style, fill=vertex-LRLRLRLR, text=text-LRLRLRLR] (node53) at (30,0.5672377983345323) {};
\node[node_style, fill=vertex-LRLRLRLL, text=text-LRLRLRLL] (node52) at (30,0.5990284824466628) {};
\node[node_style, fill=vertex-LRLRLRL, text=text-LRLRLRL] (node51) at (28.9097128984883,0.5771025713057278) {$z_{74}$};
\node[node_style, fill=vertex-LRLRLR, text=text-LRLRLR] (node50) at (18.2730451176435,0.5573730253633367) {$z_{44}$};
\node[node_style, fill=vertex-LRLRLLR, text=text-LRLRLLR] (node49) at (30,0.634898719053089) {};
\node[node_style, fill=vertex-LRLRLLL, text=text-LRLRLLL] (node48) at (30,0.6539558063025448) {};
\node[node_style, fill=vertex-LRLRLL, text=text-LRLRLL] (node47) at (27.6731548544841,0.6488430445185801) {$z_{87}$};
\node[node_style, fill=vertex-LRLRL, text=text-LRLRL] (node46) at (14.4999128697711,0.6209543935875979) {$z_{51}$};
\node[node_style, fill=vertex-LRLR, text=text-LRLR] (node45) at (7.57469162085984,0.5495018468977895) {$z_{42}$};
\node[node_style, fill=vertex-LRLLR, text=text-LRLLR] (node44) at (30,0.6821062901268649) {};
\node[node_style, fill=vertex-LRLLLR, text=text-LRLLLR] (node43) at (30,0.7220569542798285) {};
\node[node_style, fill=vertex-LRLLLLR, text=text-LRLLLLR] (node42) at (30,0.74902790350952) {};
\node[node_style, fill=vertex-LRLLLLL, text=text-LRLLLLL] (node41) at (30,0.7689329743442888) {};
\node[node_style, fill=vertex-LRLLLL, text=text-LRLLLL] (node40) at (24.9499619721022,0.7590859106266032) {$z_{33}$};
\node[node_style, fill=vertex-LRLLL, text=text-LRLLL] (node39) at (22.9592284464169,0.7389698963924368) {$z_{102}$};
\node[node_style, fill=vertex-LRLL, text=text-LRLL] (node38) at (12.2206889176002,0.7051440121672201) {$z_{4}$};
\node[node_style, fill=vertex-LRL, text=text-LRL] (node37) at (5.34959587656006,0.6590685680865096) {$z_{21}$};
\node[node_style, fill=vertex-LR, text=text-LR] (node36) at (3.28181803491129,0.45734889345629326) {$z_{13}$};
\node[node_style, fill=vertex-LLRR, text=text-LLRR] (node35) at (30,0.7917567069652724) {};
\node[node_style, fill=vertex-LLRLRRR, text=text-LLRLRRR] (node34) at (30,0.8186394355182063) {};
\node[node_style, fill=vertex-LLRLRRLR, text=text-LLRLRRLR] (node33) at (30,0.8386374031554333) {};
\node[node_style, fill=vertex-LLRLRRLL, text=text-LLRLRRLL] (node32) at (30,0.8510674789368524) {};
\node[node_style, fill=vertex-LLRLRRL, text=text-LLRLRRL] (node31) at (25.9635956659396,0.8447293111430249) {$z_{203}$};
\node[node_style, fill=vertex-LLRLRR, text=text-LLRLRR] (node30) at (17.5994378810111,0.8325454951678419) {$z_{48}$};
\node[node_style, fill=vertex-LLRLRL, text=text-LLRLRL] (node29) at (30,0.8670175003535026) {};
\node[node_style, fill=vertex-LLRLR, text=text-LLRLR] (node28) at (14.0039159951399,0.85740564673068) {$z_{54}$};
\node[node_style, fill=vertex-LLRLLRRR, text=text-LLRLLRRR] (node27) at (30,0.8830164592255905) {};
\node[node_style, fill=vertex-LLRLLRRL, text=text-LLRLLRRL] (node26) at (30,0.897563552023884) {};
\node[node_style, fill=vertex-LLRLLRR, text=text-LLRLLRR] (node25) at (27.0685667989319,0.889403564474856) {$z_{73}$};
\node[node_style, fill=vertex-LLRLLRLR, text=text-LLRLLRLR] (node24) at (30,0.9167182947094366) {};
\node[node_style, fill=vertex-LLRLLRLL, text=text-LLRLLRLL] (node23) at (30,0.9340610547735977) {};
\node[node_style, fill=vertex-LLRLLRL, text=text-LLRLLRL] (node22) at (20.4110002041305,0.9277130498459609) {$z_{122}$};
\node[node_style, fill=vertex-LLRLLR, text=text-LLRLLR] (node21) at (16.8721139144636,0.9057235395729122) {$z_{63}$};
\node[node_style, fill=vertex-LLRLLLR, text=text-LLRLLLR] (node20) at (30,0.9418027212785761) {};
\node[node_style, fill=vertex-LLRLLLL, text=text-LLRLLLL] (node19) at (30,0.946408832174903) {};
\node[node_style, fill=vertex-LLRLLL, text=text-LLRLLL] (node18) at (26.0123802079731,0.9431963828559177) {$z_{19}$};
\node[node_style, fill=vertex-LLRLL, text=text-LLRLL] (node17) at (10.1786550773388,0.9404090597012346) {$z_{24}$};
\node[node_style, fill=vertex-LLRL, text=text-LLRL] (node16) at (9.68546928116901,0.876629353976325) {$z_{56}$};
\node[node_style, fill=vertex-LLR, text=text-LLR] (node15) at (6.71647037323622,0.8047333758685706) {$z_{34}$};
\node[node_style, fill=vertex-LLLRRR, text=text-LLLRRR] (node14) at (30,0.9529550910739552) {};
\node[node_style, fill=vertex-LLLRRL, text=text-LLLRRL] (node13) at (30,0.9612024900595554) {$z_{27}$};
\node[node_style, fill=vertex-LLLRR, text=text-LLLRR] (node12) at (22.6436917169764,0.956288900654022) {$z_{23}$};
\node[node_style, fill=vertex-LLLRL, text=text-LLLRL] (node11) at (30,0.9883161927476714) {$z_{277}$};
\node[node_style, fill=vertex-LLLR, text=text-LLLR] (node10) at (10.2404385600867,0.9755561315522409) {$z_{35}$};
\node[node_style, fill=vertex-LLLLR, text=text-LLLLR] (node9) at (30,0.993815931819102) {};
\node[node_style, fill=vertex-LLLLLR, text=text-LLLLLR] (node8) at (30,0.997862574609754) {};
\node[node_style, fill=vertex-LLLLLL, text=text-LLLLLL] (node7) at (30,0.999375981476383) {};
\node[node_style, fill=vertex-LLLLL, text=text-LLLLL] (node6) at (18.8671433922190,0.998751962952766) {$z_{492}$};
\node[node_style, fill=vertex-LLLL, text=text-LLLL] (node5) at (15.0303521945341,0.9969731862667421) {$z_{398}$};
\node[node_style, fill=vertex-LLL, text=text-LLL] (node4) at (8.32401638665374,0.9906586773714617) {$z_{9}$};
\node[node_style, fill=vertex-LL, text=text-LL] (node3) at (3.11373725847777,0.9496212814938884) {$z_{7}$};
\node[node_style, fill=vertex-L, text=text-L] (node2) at (1.49534878122122,0.7787800380619743) {$z_{2}$};
\node[node_style, fill=vertex-root, text=text-root] (node1) at (1.00000000000000,0.22000131666063394) {$z_{1}$};

\begin{scope}[on background layer]
\clipcommand


\draw[my edge style] (node6) -- (node7);
\draw[my edge style] (node6) -- (node8);
\draw[my edge style] (node5) -- (node6);
\draw[my edge style] (node5) -- (node9);
\draw[my edge style] (node4) -- (node5);
\draw[my edge style] (node10) -- (node11);
\draw[my edge style] (node12) -- (node13);
\draw[my edge style] (node12) -- (node14);
\draw[my edge style] (node10) -- (node12);
\draw[my edge style] (node4) -- (node10);
\draw[my edge style] (node3) -- (node4);
\draw[my edge style] (node18) -- (node19);
\draw[my edge style] (node18) -- (node20);
\draw[my edge style] (node17) -- (node18);
\draw[my edge style] (node22) -- (node23);
\draw[my edge style] (node22) -- (node24);
\draw[my edge style] (node21) -- (node22);
\draw[my edge style] (node25) -- (node26);
\draw[my edge style] (node25) -- (node27);
\draw[my edge style] (node21) -- (node25);
\draw[my edge style] (node17) -- (node21);
\draw[my edge style] (node16) -- (node17);
\draw[my edge style] (node28) -- (node29);
\draw[my edge style] (node31) -- (node32);
\draw[my edge style] (node31) -- (node33);
\draw[my edge style] (node30) -- (node31);
\draw[my edge style] (node30) -- (node34);
\draw[my edge style] (node28) -- (node30);
\draw[my edge style] (node16) -- (node28);
\draw[my edge style] (node15) -- (node16);
\draw[my edge style] (node15) -- (node35);
\draw[my edge style] (node3) -- (node15);
\draw[my edge style] (node2) -- (node3);
\draw[my edge style] (node40) -- (node41);
\draw[my edge style] (node40) -- (node42);
\draw[my edge style] (node39) -- (node40);
\draw[my edge style] (node39) -- (node43);
\draw[my edge style] (node38) -- (node39);
\draw[my edge style] (node38) -- (node44);
\draw[my edge style] (node37) -- (node38);
\draw[my edge style] (node47) -- (node48);
\draw[my edge style] (node47) -- (node49);
\draw[my edge style] (node46) -- (node47);
\draw[my edge style] (node51) -- (node52);
\draw[my edge style] (node51) -- (node53);
\draw[my edge style] (node50) -- (node51);
\draw[my edge style] (node50) -- (node54);
\draw[my edge style] (node46) -- (node50);
\draw[my edge style] (node45) -- (node46);
\draw[my edge style] (node57) -- (node58);
\draw[my edge style] (node57) -- (node59);
\draw[my edge style] (node56) -- (node57);
\draw[my edge style] (node56) -- (node60);
\draw[my edge style] (node55) -- (node56);
\draw[my edge style] (node55) -- (node61);
\draw[my edge style] (node45) -- (node55);
\draw[my edge style] (node37) -- (node45);
\draw[my edge style] (node36) -- (node37);
\draw[my edge style] (node64) -- (node65);
\draw[my edge style] (node64) -- (node66);
\draw[my edge style] (node63) -- (node64);
\draw[my edge style] (node63) -- (node67);
\draw[my edge style] (node62) -- (node63);
\draw[my edge style] (node69) -- (node70);
\draw[my edge style] (node69) -- (node71);
\draw[my edge style] (node68) -- (node69);
\draw[my edge style] (node74) -- (node75);
\draw[my edge style] (node74) -- (node76);
\draw[my edge style] (node73) -- (node74);
\draw[my edge style] (node73) -- (node77);
\draw[my edge style] (node72) -- (node73);
\draw[my edge style] (node78) -- (node79);
\draw[my edge style] (node78) -- (node80);
\draw[my edge style] (node72) -- (node78);
\draw[my edge style] (node68) -- (node72);
\draw[my edge style] (node62) -- (node68);
\draw[my edge style] (node36) -- (node62);
\draw[my edge style] (node2) -- (node36);
\draw[my edge style] (node1) -- (node2);
\draw[my edge style] (node83) -- (node84);
\draw[my edge style] (node85) -- (node86);
\draw[my edge style] (node85) -- (node87);
\draw[my edge style] (node83) -- (node85);
\draw[my edge style] (node82) -- (node83);
\draw[my edge style] (node91) -- (node92);
\draw[my edge style] (node91) -- (node93);
\draw[my edge style] (node90) -- (node91);
\draw[my edge style] (node90) -- (node94);
\draw[my edge style] (node89) -- (node90);
\draw[my edge style] (node89) -- (node95);
\draw[my edge style] (node88) -- (node89);
\draw[my edge style] (node97) -- (node98);
\draw[my edge style] (node97) -- (node99);
\draw[my edge style] (node96) -- (node97);
\draw[my edge style] (node96) -- (node100);
\draw[my edge style] (node88) -- (node96);
\draw[my edge style] (node82) -- (node88);
\draw[my edge style] (node81) -- (node82);
\draw[my edge style] (node103) -- (node104);
\draw[my edge style] (node103) -- (node105);
\draw[my edge style] (node102) -- (node103);
\draw[my edge style] (node102) -- (node106);
\draw[my edge style] (node101) -- (node102);
\draw[my edge style] (node108) -- (node109);
\draw[my edge style] (node108) -- (node110);
\draw[my edge style] (node107) -- (node108);
\draw[my edge style] (node112) -- (node113);
\draw[my edge style] (node112) -- (node114);
\draw[my edge style] (node111) -- (node112);
\draw[my edge style] (node111) -- (node115);
\draw[my edge style] (node107) -- (node111);
\draw[my edge style] (node101) -- (node107);
\draw[my edge style] (node81) -- (node101);
\draw[my edge style] (node1) -- (node81);
\end{scope}




==> figures/autogenerated/cusp-direction-cdf-content.tex <==
%% Auto-generated by cusp_direction_cdf_export.py -- do not edit.
% Empirical CDF of cusp directions z in [0,1], per radial shell R=t^{1/4}.  n=10^6, N_real=2000.
%% Box: x=z in [0,1], y=F_emp in [0,1]; coords in [0,1]^2.
%% shell R in [5,10]: N=18879
\draw[resA] plot coordinates {(0.0000,0.0000) (0.0050,0.0322) (0.0100,0.0533) (0.0150,0.0683) (0.0200,0.0810) (0.0250,0.0935) (0.0300,0.1031) (0.0350,0.1128) (0.0400,0.1207) (0.0450,0.1291) (0.0500,0.1375) (0.0550,0.1440) (0.0600,0.1502) (0.0650,0.1564) (0.0700,0.1627) (0.0750,0.1689) (0.0800,0.1745) (0.0850,0.1806) (0.0900,0.1857) (0.0950,0.1915) (0.1000,0.1969) (0.1050,0.2017) (0.1100,0.2065) (0.1150,0.2122) (0.1200,0.2171) (0.1250,0.2224) (0.1300,0.2270) (0.1350,0.2318) (0.1400,0.2356) (0.1450,0.2404) (0.1500,0.2447) (0.1550,0.2495) (0.1600,0.2544) (0.1650,0.2592) (0.1700,0.2635) (0.1750,0.2686) (0.1800,0.2717) (0.1850,0.2764) (0.1900,0.2807) (0.1950,0.2844) (0.2000,0.2889) (0.2050,0.2935) (0.2100,0.2970) (0.2150,0.3009) (0.2200,0.3058) (0.2250,0.3093) (0.2300,0.3140) (0.2350,0.3177) (0.2400,0.3215) (0.2450,0.3260) (0.2500,0.3294) (0.2550,0.3335) (0.2600,0.3359) (0.2650,0.3394) (0.2700,0.3435) (0.2750,0.3468) (0.2800,0.3509) (0.2850,0.3536) (0.2900,0.3571) (0.2950,0.3605) (0.3000,0.3632) (0.3050,0.3680) (0.3100,0.3713) (0.3150,0.3746) (0.3200,0.3785) (0.3250,0.3826) (0.3300,0.3861) (0.3350,0.3899) (0.3400,0.3935) (0.3450,0.3964) (0.3500,0.3997) (0.3550,0.4021) (0.3600,0.4059) (0.3650,0.4093) (0.3700,0.4124) (0.3750,0.4158) (0.3800,0.4190) (0.3850,0.4224) (0.3900,0.4258) (0.3950,0.4294) (0.4000,0.4328) (0.4050,0.4358) (0.4100,0.4387) (0.4150,0.4414) (0.4200,0.4456) (0.4250,0.4491) (0.4300,0.4522) (0.4350,0.4556) (0.4400,0.4589) (0.4450,0.4616) (0.4500,0.4646) (0.4550,0.4681) (0.4600,0.4716) (0.4650,0.4744) (0.4700,0.4784) (0.4750,0.4820) (0.4800,0.4859) (0.4850,0.4896) (0.4900,0.4925) (0.4950,0.4954) (0.5000,0.4990) (0.5050,0.5020) (0.5100,0.5058) (0.5150,0.5090) (0.5200,0.5120) (0.5250,0.5154) (0.5300,0.5184) (0.5350,0.5218) (0.5400,0.5252) (0.5450,0.5282) (0.5500,0.5318) (0.5550,0.5346) (0.5600,0.5371) (0.5650,0.5413) (0.5700,0.5447) (0.5750,0.5476) (0.5800,0.5509) (0.5850,0.5543) (0.5900,0.5579) (0.5950,0.5615) (0.6000,0.5646) (0.6050,0.5681) (0.6100,0.5715) (0.6150,0.5744) (0.6200,0.5775) (0.6250,0.5811) (0.6300,0.5846) (0.6350,0.5875) (0.6400,0.5910) (0.6450,0.5946) (0.6500,0.5977) (0.6550,0.6013) (0.6600,0.6052) (0.6650,0.6089) (0.6700,0.6126) (0.6750,0.6159) (0.6800,0.6195) (0.6850,0.6230) (0.6900,0.6263) (0.6950,0.6297) (0.7000,0.6328) (0.7050,0.6357) (0.7100,0.6396) (0.7150,0.6442) (0.7200,0.6482) (0.7250,0.6518) (0.7300,0.6553) (0.7350,0.6583) (0.7400,0.6620) (0.7450,0.6656) (0.7500,0.6700) (0.7550,0.6733) (0.7600,0.6785) (0.7650,0.6827) (0.7700,0.6874) (0.7750,0.6911) (0.7800,0.6952) (0.7850,0.6987) (0.7900,0.7023) (0.7950,0.7062) (0.8000,0.7101) (0.8050,0.7135) (0.8100,0.7172) (0.8150,0.7215) (0.8200,0.7256) (0.8250,0.7298) (0.8300,0.7344) (0.8350,0.7388) (0.8400,0.7429) (0.8450,0.7469) (0.8500,0.7522) (0.8550,0.7569) (0.8600,0.7622) (0.8650,0.7674) (0.8700,0.7721) (0.8750,0.7774) (0.8800,0.7818) (0.8850,0.7859) (0.8900,0.7916) (0.8950,0.7971) (0.9000,0.8027) (0.9050,0.8085) (0.9100,0.8151) (0.9150,0.8212) (0.9200,0.8274) (0.9250,0.8330) (0.9300,0.8404) (0.9350,0.8465) (0.9400,0.8522) (0.9450,0.8595) (0.9500,0.8659) (0.9550,0.8739) (0.9600,0.8814) (0.9650,0.8901) (0.9700,0.8997) (0.9750,0.9086) (0.9800,0.9196) (0.9850,0.9332) (0.9900,0.9486) (0.9950,0.9693) (1.0000,1.0000)};
%% shell R in [10,15]: N=18841
\draw[resB] plot coordinates {(0.0000,0.0000) (0.0050,0.0387) (0.0100,0.0599) (0.0150,0.0726) (0.0200,0.0848) (0.0250,0.0955) (0.0300,0.1054) (0.0350,0.1149) (0.0400,0.1222) (0.0450,0.1296) (0.0500,0.1377) (0.0550,0.1454) (0.0600,0.1536) (0.0650,0.1601) (0.0700,0.1660) (0.0750,0.1721) (0.0800,0.1776) (0.0850,0.1838) (0.0900,0.1893) (0.0950,0.1953) (0.1000,0.2004) (0.1050,0.2062) (0.1100,0.2106) (0.1150,0.2156) (0.1200,0.2213) (0.1250,0.2263) (0.1300,0.2307) (0.1350,0.2367) (0.1400,0.2420) (0.1450,0.2472) (0.1500,0.2521) (0.1550,0.2570) (0.1600,0.2603) (0.1650,0.2652) (0.1700,0.2694) (0.1750,0.2738) (0.1800,0.2772) (0.1850,0.2808) (0.1900,0.2848) (0.1950,0.2889) (0.2000,0.2933) (0.2050,0.2970) (0.2100,0.3008) (0.2150,0.3048) (0.2200,0.3090) (0.2250,0.3135) (0.2300,0.3168) (0.2350,0.3202) (0.2400,0.3242) (0.2450,0.3272) (0.2500,0.3308) (0.2550,0.3352) (0.2600,0.3393) (0.2650,0.3423) (0.2700,0.3459) (0.2750,0.3491) (0.2800,0.3530) (0.2850,0.3573) (0.2900,0.3597) (0.2950,0.3635) (0.3000,0.3672) (0.3050,0.3712) (0.3100,0.3743) (0.3150,0.3782) (0.3200,0.3823) (0.3250,0.3859) (0.3300,0.3889) (0.3350,0.3929) (0.3400,0.3959) (0.3450,0.3998) (0.3500,0.4033) (0.3550,0.4062) (0.3600,0.4101) (0.3650,0.4132) (0.3700,0.4165) (0.3750,0.4203) (0.3800,0.4233) (0.3850,0.4271) (0.3900,0.4298) (0.3950,0.4329) (0.4000,0.4359) (0.4050,0.4395) (0.4100,0.4424) (0.4150,0.4462) (0.4200,0.4497) (0.4250,0.4529) (0.4300,0.4558) (0.4350,0.4587) (0.4400,0.4618) (0.4450,0.4648) (0.4500,0.4678) (0.4550,0.4716) (0.4600,0.4746) (0.4650,0.4779) (0.4700,0.4805) (0.4750,0.4832) (0.4800,0.4865) (0.4850,0.4902) (0.4900,0.4933) (0.4950,0.4965) (0.5000,0.4993) (0.5050,0.5026) (0.5100,0.5061) (0.5150,0.5094) (0.5200,0.5127) (0.5250,0.5166) (0.5300,0.5209) (0.5350,0.5247) (0.5400,0.5276) (0.5450,0.5311) (0.5500,0.5347) (0.5550,0.5380) (0.5600,0.5411) (0.5650,0.5439) (0.5700,0.5469) (0.5750,0.5498) (0.5800,0.5523) (0.5850,0.5559) (0.5900,0.5599) (0.5950,0.5637) (0.6000,0.5676) (0.6050,0.5713) (0.6100,0.5746) (0.6150,0.5788) (0.6200,0.5826) (0.6250,0.5859) (0.6300,0.5891) (0.6350,0.5924) (0.6400,0.5954) (0.6450,0.5980) (0.6500,0.6015) (0.6550,0.6047) (0.6600,0.6085) (0.6650,0.6123) (0.6700,0.6153) (0.6750,0.6182) (0.6800,0.6219) (0.6850,0.6247) (0.6900,0.6284) (0.6950,0.6320) (0.7000,0.6356) (0.7050,0.6395) (0.7100,0.6427) (0.7150,0.6465) (0.7200,0.6499) (0.7250,0.6543) (0.7300,0.6582) (0.7350,0.6619) (0.7400,0.6660) (0.7450,0.6697) (0.7500,0.6736) (0.7550,0.6770) (0.7600,0.6807) (0.7650,0.6848) (0.7700,0.6879) (0.7750,0.6916) (0.7800,0.6954) (0.7850,0.6994) (0.7900,0.7039) (0.7950,0.7073) (0.8000,0.7108) (0.8050,0.7148) (0.8100,0.7196) (0.8150,0.7231) (0.8200,0.7275) (0.8250,0.7318) (0.8300,0.7362) (0.8350,0.7410) (0.8400,0.7452) (0.8450,0.7498) (0.8500,0.7543) (0.8550,0.7585) (0.8600,0.7635) (0.8650,0.7676) (0.8700,0.7719) (0.8750,0.7764) (0.8800,0.7807) (0.8850,0.7860) (0.8900,0.7910) (0.8950,0.7956) (0.9000,0.8012) (0.9050,0.8066) (0.9100,0.8114) (0.9150,0.8168) (0.9200,0.8229) (0.9250,0.8294) (0.9300,0.8342) (0.9350,0.8405) (0.9400,0.8463) (0.9450,0.8537) (0.9500,0.8613) (0.9550,0.8682) (0.9600,0.8763) (0.9650,0.8846) (0.9700,0.8944) (0.9750,0.9037) (0.9800,0.9147) (0.9850,0.9282) (0.9900,0.9430) (0.9950,0.9632) (1.0000,1.0000)};
%% shell R in [15,20]: N=18573
\draw[resC] plot coordinates {(0.0000,0.0000) (0.0050,0.0383) (0.0100,0.0539) (0.0150,0.0692) (0.0200,0.0823) (0.0250,0.0929) (0.0300,0.1019) (0.0350,0.1116) (0.0400,0.1186) (0.0450,0.1266) (0.0500,0.1341) (0.0550,0.1406) (0.0600,0.1477) (0.0650,0.1549) (0.0700,0.1617) (0.0750,0.1673) (0.0800,0.1733) (0.0850,0.1786) (0.0900,0.1840) (0.0950,0.1891) (0.1000,0.1934) (0.1050,0.1994) (0.1100,0.2041) (0.1150,0.2089) (0.1200,0.2143) (0.1250,0.2198) (0.1300,0.2252) (0.1350,0.2299) (0.1400,0.2344) (0.1450,0.2386) (0.1500,0.2431) (0.1550,0.2468) (0.1600,0.2511) (0.1650,0.2557) (0.1700,0.2600) (0.1750,0.2643) (0.1800,0.2693) (0.1850,0.2730) (0.1900,0.2771) (0.1950,0.2804) (0.2000,0.2851) (0.2050,0.2891) (0.2100,0.2928) (0.2150,0.2968) (0.2200,0.3010) (0.2250,0.3051) (0.2300,0.3088) (0.2350,0.3128) (0.2400,0.3178) (0.2450,0.3221) (0.2500,0.3264) (0.2550,0.3302) (0.2600,0.3343) (0.2650,0.3383) (0.2700,0.3416) (0.2750,0.3452) (0.2800,0.3486) (0.2850,0.3528) (0.2900,0.3561) (0.2950,0.3596) (0.3000,0.3628) (0.3050,0.3659) (0.3100,0.3693) (0.3150,0.3720) (0.3200,0.3758) (0.3250,0.3791) (0.3300,0.3827) (0.3350,0.3867) (0.3400,0.3897) (0.3450,0.3938) (0.3500,0.3974) (0.3550,0.4013) (0.3600,0.4046) (0.3650,0.4078) (0.3700,0.4111) (0.3750,0.4140) (0.3800,0.4175) (0.3850,0.4211) (0.3900,0.4245) (0.3950,0.4277) (0.4000,0.4305) (0.4050,0.4353) (0.4100,0.4382) (0.4150,0.4413) (0.4200,0.4445) (0.4250,0.4477) (0.4300,0.4509) (0.4350,0.4546) (0.4400,0.4581) (0.4450,0.4615) (0.4500,0.4648) (0.4550,0.4684) (0.4600,0.4719) (0.4650,0.4748) (0.4700,0.4780) (0.4750,0.4808) (0.4800,0.4841) (0.4850,0.4876) (0.4900,0.4906) (0.4950,0.4943) (0.5000,0.4970) (0.5050,0.5001) (0.5100,0.5037) (0.5150,0.5071) (0.5200,0.5109) (0.5250,0.5142) (0.5300,0.5170) (0.5350,0.5199) (0.5400,0.5227) (0.5450,0.5264) (0.5500,0.5297) (0.5550,0.5335) (0.5600,0.5360) (0.5650,0.5396) (0.5700,0.5429) (0.5750,0.5457) (0.5800,0.5492) (0.5850,0.5531) (0.5900,0.5561) (0.5950,0.5593) (0.6000,0.5626) (0.6050,0.5659) (0.6100,0.5695) (0.6150,0.5731) (0.6200,0.5769) (0.6250,0.5806) (0.6300,0.5839) (0.6350,0.5877) (0.6400,0.5913) (0.6450,0.5947) (0.6500,0.5983) (0.6550,0.6014) (0.6600,0.6042) (0.6650,0.6077) (0.6700,0.6114) (0.6750,0.6152) (0.6800,0.6189) (0.6850,0.6231) (0.6900,0.6268) (0.6950,0.6298) (0.7000,0.6330) (0.7050,0.6361) (0.7100,0.6391) (0.7150,0.6424) (0.7200,0.6463) (0.7250,0.6498) (0.7300,0.6536) (0.7350,0.6570) (0.7400,0.6610) (0.7450,0.6644) (0.7500,0.6679) (0.7550,0.6717) (0.7600,0.6752) (0.7650,0.6791) (0.7700,0.6831) (0.7750,0.6867) (0.7800,0.6910) (0.7850,0.6958) (0.7900,0.6986) (0.7950,0.7030) (0.8000,0.7075) (0.8050,0.7114) (0.8100,0.7161) (0.8150,0.7201) (0.8200,0.7256) (0.8250,0.7301) (0.8300,0.7352) (0.8350,0.7394) (0.8400,0.7444) (0.8450,0.7486) (0.8500,0.7523) (0.8550,0.7571) (0.8600,0.7612) (0.8650,0.7663) (0.8700,0.7712) (0.8750,0.7752) (0.8800,0.7794) (0.8850,0.7840) (0.8900,0.7894) (0.8950,0.7938) (0.9000,0.7984) (0.9050,0.8040) (0.9100,0.8098) (0.9150,0.8150) (0.9200,0.8207) (0.9250,0.8266) (0.9300,0.8333) (0.9350,0.8397) (0.9400,0.8467) (0.9450,0.8538) (0.9500,0.8605) (0.9550,0.8683) (0.9600,0.8752) (0.9650,0.8845) (0.9700,0.8937) (0.9750,0.9041) (0.9800,0.9144) (0.9850,0.9271) (0.9900,0.9403) (0.9950,0.9582) (1.0000,1.0000)};
%% shell R in [20,25]: N=18560
\draw[resD] plot coordinates {(0.0000,0.0000) (0.0050,0.0425) (0.0100,0.0616) (0.0150,0.0760) (0.0200,0.0874) (0.0250,0.0973) (0.0300,0.1067) (0.0350,0.1157) (0.0400,0.1246) (0.0450,0.1319) (0.0500,0.1394) (0.0550,0.1473) (0.0600,0.1539) (0.0650,0.1603) (0.0700,0.1665) (0.0750,0.1732) (0.0800,0.1794) (0.0850,0.1856) (0.0900,0.1916) (0.0950,0.1978) (0.1000,0.2034) (0.1050,0.2091) (0.1100,0.2137) (0.1150,0.2183) (0.1200,0.2231) (0.1250,0.2281) (0.1300,0.2335) (0.1350,0.2377) (0.1400,0.2427) (0.1450,0.2474) (0.1500,0.2516) (0.1550,0.2562) (0.1600,0.2606) (0.1650,0.2643) (0.1700,0.2685) (0.1750,0.2724) (0.1800,0.2766) (0.1850,0.2814) (0.1900,0.2856) (0.1950,0.2895) (0.2000,0.2937) (0.2050,0.2985) (0.2100,0.3019) (0.2150,0.3063) (0.2200,0.3099) (0.2250,0.3138) (0.2300,0.3166) (0.2350,0.3205) (0.2400,0.3244) (0.2450,0.3276) (0.2500,0.3319) (0.2550,0.3354) (0.2600,0.3395) (0.2650,0.3430) (0.2700,0.3472) (0.2750,0.3512) (0.2800,0.3548) (0.2850,0.3586) (0.2900,0.3626) (0.2950,0.3659) (0.3000,0.3695) (0.3050,0.3723) (0.3100,0.3765) (0.3150,0.3798) (0.3200,0.3830) (0.3250,0.3854) (0.3300,0.3886) (0.3350,0.3920) (0.3400,0.3957) (0.3450,0.3991) (0.3500,0.4027) (0.3550,0.4058) (0.3600,0.4092) (0.3650,0.4129) (0.3700,0.4158) (0.3750,0.4195) (0.3800,0.4229) (0.3850,0.4265) (0.3900,0.4303) (0.3950,0.4341) (0.4000,0.4373) (0.4050,0.4408) (0.4100,0.4441) (0.4150,0.4472) (0.4200,0.4508) (0.4250,0.4543) (0.4300,0.4580) (0.4350,0.4605) (0.4400,0.4640) (0.4450,0.4670) (0.4500,0.4709) (0.4550,0.4743) (0.4600,0.4777) (0.4650,0.4808) (0.4700,0.4836) (0.4750,0.4870) (0.4800,0.4905) (0.4850,0.4939) (0.4900,0.4973) (0.4950,0.5018) (0.5000,0.5059) (0.5050,0.5096) (0.5100,0.5125) (0.5150,0.5160) (0.5200,0.5197) (0.5250,0.5229) (0.5300,0.5264) (0.5350,0.5299) (0.5400,0.5331) (0.5450,0.5364) (0.5500,0.5391) (0.5550,0.5422) (0.5600,0.5454) (0.5650,0.5489) (0.5700,0.5522) (0.5750,0.5559) (0.5800,0.5594) (0.5850,0.5634) (0.5900,0.5673) (0.5950,0.5698) (0.6000,0.5722) (0.6050,0.5755) (0.6100,0.5783) (0.6150,0.5808) (0.6200,0.5842) (0.6250,0.5880) (0.6300,0.5912) (0.6350,0.5946) (0.6400,0.5979) (0.6450,0.6017) (0.6500,0.6050) (0.6550,0.6082) (0.6600,0.6115) (0.6650,0.6149) (0.6700,0.6187) (0.6750,0.6226) (0.6800,0.6260) (0.6850,0.6297) (0.6900,0.6336) (0.6950,0.6366) (0.7000,0.6405) (0.7050,0.6436) (0.7100,0.6478) (0.7150,0.6515) (0.7200,0.6551) (0.7250,0.6586) (0.7300,0.6628) (0.7350,0.6667) (0.7400,0.6707) (0.7450,0.6742) (0.7500,0.6778) (0.7550,0.6810) (0.7600,0.6846) (0.7650,0.6888) (0.7700,0.6929) (0.7750,0.6966) (0.7800,0.7003) (0.7850,0.7039) (0.7900,0.7071) (0.7950,0.7109) (0.8000,0.7149) (0.8050,0.7191) (0.8100,0.7227) (0.8150,0.7266) (0.8200,0.7309) (0.8250,0.7354) (0.8300,0.7391) (0.8350,0.7435) (0.8400,0.7473) (0.8450,0.7517) (0.8500,0.7569) (0.8550,0.7616) (0.8600,0.7662) (0.8650,0.7705) (0.8700,0.7749) (0.8750,0.7798) (0.8800,0.7850) (0.8850,0.7895) (0.8900,0.7955) (0.8950,0.8004) (0.9000,0.8050) (0.9050,0.8096) (0.9100,0.8148) (0.9150,0.8199) (0.9200,0.8259) (0.9250,0.8320) (0.9300,0.8387) (0.9350,0.8448) (0.9400,0.8518) (0.9450,0.8578) (0.9500,0.8656) (0.9550,0.8731) (0.9600,0.8812) (0.9650,0.8890) (0.9700,0.8977) (0.9750,0.9054) (0.9800,0.9166) (0.9850,0.9281) (0.9900,0.9431) (0.9950,0.9595) (1.0000,1.0000)};
%% shell R in [25,30]: N=18626
\draw[resE] plot coordinates {(0.0000,0.0000) (0.0050,0.0409) (0.0100,0.0606) (0.0150,0.0758) (0.0200,0.0872) (0.0250,0.0980) (0.0300,0.1075) (0.0350,0.1168) (0.0400,0.1253) (0.0450,0.1331) (0.0500,0.1410) (0.0550,0.1478) (0.0600,0.1553) (0.0650,0.1611) (0.0700,0.1671) (0.0750,0.1733) (0.0800,0.1792) (0.0850,0.1843) (0.0900,0.1903) (0.0950,0.1962) (0.1000,0.2011) (0.1050,0.2060) (0.1100,0.2115) (0.1150,0.2169) (0.1200,0.2214) (0.1250,0.2269) (0.1300,0.2314) (0.1350,0.2353) (0.1400,0.2399) (0.1450,0.2449) (0.1500,0.2487) (0.1550,0.2536) (0.1600,0.2572) (0.1650,0.2618) (0.1700,0.2658) (0.1750,0.2695) (0.1800,0.2734) (0.1850,0.2772) (0.1900,0.2811) (0.1950,0.2855) (0.2000,0.2892) (0.2050,0.2934) (0.2100,0.2978) (0.2150,0.3010) (0.2200,0.3044) (0.2250,0.3076) (0.2300,0.3116) (0.2350,0.3158) (0.2400,0.3193) (0.2450,0.3233) (0.2500,0.3270) (0.2550,0.3316) (0.2600,0.3350) (0.2650,0.3385) (0.2700,0.3420) (0.2750,0.3459) (0.2800,0.3497) (0.2850,0.3531) (0.2900,0.3565) (0.2950,0.3598) (0.3000,0.3634) (0.3050,0.3668) (0.3100,0.3699) (0.3150,0.3735) (0.3200,0.3776) (0.3250,0.3810) (0.3300,0.3845) (0.3350,0.3870) (0.3400,0.3905) (0.3450,0.3943) (0.3500,0.3976) (0.3550,0.4022) (0.3600,0.4063) (0.3650,0.4095) (0.3700,0.4132) (0.3750,0.4168) (0.3800,0.4211) (0.3850,0.4245) (0.3900,0.4280) (0.3950,0.4309) (0.4000,0.4343) (0.4050,0.4377) (0.4100,0.4410) (0.4150,0.4445) (0.4200,0.4479) (0.4250,0.4510) (0.4300,0.4550) (0.4350,0.4580) (0.4400,0.4619) (0.4450,0.4651) (0.4500,0.4683) (0.4550,0.4712) (0.4600,0.4744) (0.4650,0.4781) (0.4700,0.4813) (0.4750,0.4849) (0.4800,0.4882) (0.4850,0.4919) (0.4900,0.4947) (0.4950,0.4982) (0.5000,0.5014) (0.5050,0.5045) (0.5100,0.5082) (0.5150,0.5115) (0.5200,0.5142) (0.5250,0.5177) (0.5300,0.5213) (0.5350,0.5248) (0.5400,0.5289) (0.5450,0.5324) (0.5500,0.5357) (0.5550,0.5382) (0.5600,0.5418) (0.5650,0.5446) (0.5700,0.5485) (0.5750,0.5522) (0.5800,0.5552) (0.5850,0.5583) (0.5900,0.5609) (0.5950,0.5640) (0.6000,0.5668) (0.6050,0.5695) (0.6100,0.5730) (0.6150,0.5762) (0.6200,0.5798) (0.6250,0.5832) (0.6300,0.5868) (0.6350,0.5893) (0.6400,0.5926) (0.6450,0.5957) (0.6500,0.5991) (0.6550,0.6029) (0.6600,0.6059) (0.6650,0.6095) (0.6700,0.6127) (0.6750,0.6166) (0.6800,0.6198) (0.6850,0.6229) (0.6900,0.6269) (0.6950,0.6312) (0.7000,0.6354) (0.7050,0.6394) (0.7100,0.6427) (0.7150,0.6468) (0.7200,0.6501) (0.7250,0.6531) (0.7300,0.6568) (0.7350,0.6601) (0.7400,0.6637) (0.7450,0.6673) (0.7500,0.6714) (0.7550,0.6754) (0.7600,0.6793) (0.7650,0.6823) (0.7700,0.6861) (0.7750,0.6899) (0.7800,0.6941) (0.7850,0.6981) (0.7900,0.7021) (0.7950,0.7057) (0.8000,0.7102) (0.8050,0.7141) (0.8100,0.7188) (0.8150,0.7225) (0.8200,0.7260) (0.8250,0.7303) (0.8300,0.7347) (0.8350,0.7387) (0.8400,0.7428) (0.8450,0.7466) (0.8500,0.7515) (0.8550,0.7564) (0.8600,0.7606) (0.8650,0.7657) (0.8700,0.7708) (0.8750,0.7765) (0.8800,0.7814) (0.8850,0.7863) (0.8900,0.7913) (0.8950,0.7964) (0.9000,0.8007) (0.9050,0.8068) (0.9100,0.8121) (0.9150,0.8178) (0.9200,0.8242) (0.9250,0.8303) (0.9300,0.8363) (0.9350,0.8421) (0.9400,0.8495) (0.9450,0.8556) (0.9500,0.8621) (0.9550,0.8698) (0.9600,0.8766) (0.9650,0.8836) (0.9700,0.8931) (0.9750,0.9016) (0.9800,0.9128) (0.9850,0.9235) (0.9900,0.9384) (0.9950,0.9569) (1.0000,1.0000)};


==> figures/autogenerated/cusp-markers-LSVK-ultra2.tex <==
% Autogenerated overlay: cusp (root-bifurcation) markers for
% fig:cusp-forest, matching the LSVK ultra2 forest realization.
%
% One marker is placed at the cusp of each visible tree (wedge),
% via \cuspX{x}{y} (defined in the figure wrapper, which draws a
% red cross with a white casing so it stays visible on any wedge).
% By cor:cusp-min-entry the cusp box is the tree's minimum-entry
% box, i.e. its root bifurcation; coordinates are the 'French
% coordinates' of that bifurcation.
%
% Data source: data/annotated_tree_seed123.json in trees-SageMath
%  .
% The region <-> cusp matching is by the L/R path string, which
% equals the vertex-<PATH> fill-colour name of each wedge in
% jdt_tree_interface_LSVK_ultra2.tex.

\cuspX{32.4}{0.0} % RRR  cusp=(324,0)
\cuspX{2.6}{0.0} % RR  cusp=(26,0)
\cuspX{23.3}{0.5} % RRL  cusp=(233,5)
\cuspX{0.4}{0.0} % R  cusp=(4,0)
\cuspX{23.7}{1.7} % RLR  cusp=(237,17)
\cuspX{44.6}{4.2} % RLRL  cusp=(446,42)
\cuspX{4.7}{0.7} % RL  cusp=(47,7)
\cuspX{50.6}{9.1} % RLL  cusp=(506,91)
\cuspX{11.9}{3.7} % LRRRR  cusp=(119,37)
\cuspX{22.4}{7.7} % LRRRRL  cusp=(224,77)
\cuspX{51.0}{19.6} % LRRRRLL  cusp=(510,196)
\cuspX{4.4}{1.3} % LRRR  cusp=(44,13)
\cuspX{10.2}{4.5} % LRRRL  cusp=(102,45)
\cuspX{0.7}{0.6} % LRR  cusp=(7,6)
\cuspX{8.3}{5.5} % LRRL  cusp=(83,55)
\cuspX{25.4}{19.9} % LRRLL  cusp=(254,199)
\cuspX{0.6}{0.6} % LR  cusp=(6,6)
\cuspX{30.9}{32.1} % LRLRR  cusp=(309,321)
\cuspX{34.4}{37.4} % LRLRRL  cusp=(344,374)
\cuspX{3.0}{4.1} % LRLR  cusp=(30,41)
\cuspX{17.9}{24.7} % LRLRLR  cusp=(179,247)
\cuspX{9.7}{17.5} % LRLRL  cusp=(97,175)
\cuspX{1.1}{2.4} % LRL  cusp=(11,24)
\cuspX{5.0}{15.1} % LRLL  cusp=(50,151)
\cuspX{0.0}{0.2} % L  cusp=(0,2)
\cuspX{0.9}{5.2} % LLR  cusp=(9,52)
\cuspX{6.2}{38.2} % LLRLRR  cusp=(62,382)
\cuspX{3.2}{25.9} % LLRLR  cusp=(32,259)
\cuspX{1.1}{13.2} % LLRL  cusp=(11,132)
\cuspX{3.0}{41.6} % LLRLLR  cusp=(30,416)
\cuspX{1.2}{14.4} % LLRLL  cusp=(12,144)
\cuspX{0.0}{1.4} % LL  cusp=(0,14)
\cuspX{0.2}{18.6} % LLLR  cusp=(2,186)
\cuspX{0.0}{12.8} % LLL  cusp=(0,128)
\cuspX{0.0}{44.1} % LLLL  cusp=(0,441)


==> figures/autogenerated/cutoff-sweep-content.tex <==
%% Auto-generated by cutoff_sweep_tikz_export.py -- do not edit.
% N(R)=#{min(tree)<=R^4}/N_real vs R=t^{1/4}; conj: N~K*R, K=1.8684.  n=10^6, N_real=2000.
% Box: x=R in [0,31.623], y=N in [0,62.0]; coords in [0,1]^2.
\draw[theory] (0,0) -- (1.0000,0.9530);
\draw[data] plot coordinates {(0.0000,0.0000) (0.0025,0.0000) (0.0050,0.0000) (0.0075,0.0000) (0.0100,0.0000) (0.0125,0.0000) (0.0150,0.0000) (0.0175,0.0000) (0.0201,0.0000) (0.0226,0.0000) (0.0251,0.0000) (0.0276,0.0000) (0.0301,0.0000) (0.0326,0.0161) (0.0351,0.0161) (0.0376,0.0161) (0.0401,0.0161) (0.0426,0.0215) (0.0451,0.0243) (0.0476,0.0262) (0.0501,0.0280) (0.0526,0.0299) (0.0551,0.0330) (0.0576,0.0355) (0.0602,0.0378) (0.0627,0.0399) (0.0652,0.0428) (0.0677,0.0444) (0.0702,0.0476) (0.0727,0.0495) (0.0752,0.0521) (0.0777,0.0545) (0.0802,0.0568) (0.0827,0.0591) (0.0852,0.0617) (0.0877,0.0642) (0.0902,0.0666) (0.0927,0.0687) (0.0952,0.0715) (0.0977,0.0739) (0.1003,0.0764) (0.1028,0.0789) (0.1053,0.0811) (0.1078,0.0837) (0.1103,0.0861) (0.1128,0.0883) (0.1153,0.0908) (0.1178,0.0933) (0.1203,0.0957) (0.1228,0.0981) (0.1253,0.1004) (0.1278,0.1027) (0.1303,0.1052) (0.1328,0.1075) (0.1353,0.1098) (0.1378,0.1122) (0.1404,0.1147) (0.1429,0.1171) (0.1454,0.1194) (0.1479,0.1219) (0.1504,0.1244) (0.1529,0.1267) (0.1554,0.1290) (0.1579,0.1312) (0.1604,0.1336) (0.1629,0.1363) (0.1654,0.1387) (0.1679,0.1414) (0.1704,0.1438) (0.1729,0.1463) (0.1754,0.1487) (0.1779,0.1511) (0.1805,0.1536) (0.1830,0.1561) (0.1855,0.1586) (0.1880,0.1608) (0.1905,0.1631) (0.1930,0.1655) (0.1955,0.1679) (0.1980,0.1706) (0.2005,0.1729) (0.2030,0.1756) (0.2055,0.1777) (0.2080,0.1799) (0.2105,0.1822) (0.2130,0.1845) (0.2155,0.1869) (0.2180,0.1893) (0.2206,0.1917) (0.2231,0.1939) (0.2256,0.1965) (0.2281,0.1989) (0.2306,0.2011) (0.2331,0.2034) (0.2356,0.2058) (0.2381,0.2080) (0.2406,0.2106) (0.2431,0.2129) (0.2456,0.2155) (0.2481,0.2177) (0.2506,0.2205) (0.2531,0.2229) (0.2556,0.2252) (0.2581,0.2275) (0.2607,0.2301) (0.2632,0.2329) (0.2657,0.2355) (0.2682,0.2376) (0.2707,0.2401) (0.2732,0.2426) (0.2757,0.2450) (0.2782,0.2477) (0.2807,0.2500) (0.2832,0.2525) (0.2857,0.2550) (0.2882,0.2573) (0.2907,0.2597) (0.2932,0.2619) (0.2957,0.2641) (0.2982,0.2666) (0.3008,0.2688) (0.3033,0.2712) (0.3058,0.2737) (0.3083,0.2760) (0.3108,0.2784) (0.3133,0.2808) (0.3158,0.2832) (0.3183,0.2856) (0.3208,0.2879) (0.3233,0.2905) (0.3258,0.2929) (0.3283,0.2954) (0.3308,0.2977) (0.3333,0.2999) (0.3358,0.3025) (0.3383,0.3047) (0.3409,0.3067) (0.3434,0.3091) (0.3459,0.3116) (0.3484,0.3141) (0.3509,0.3166) (0.3534,0.3189) (0.3559,0.3211) (0.3584,0.3236) (0.3609,0.3263) (0.3634,0.3289) (0.3659,0.3312) (0.3684,0.3334) (0.3709,0.3359) (0.3734,0.3384) (0.3759,0.3407) (0.3784,0.3431) (0.3810,0.3456) (0.3835,0.3481) (0.3860,0.3505) (0.3885,0.3529) (0.3910,0.3554) (0.3935,0.3576) (0.3960,0.3597) (0.3985,0.3622) (0.4010,0.3647) (0.4035,0.3671) (0.4060,0.3694) (0.4085,0.3718) (0.4110,0.3744) (0.4135,0.3768) (0.4160,0.3792) (0.4185,0.3816) (0.4211,0.3841) (0.4236,0.3866) (0.4261,0.3889) (0.4286,0.3914) (0.4311,0.3936) (0.4336,0.3960) (0.4361,0.3984) (0.4386,0.4009) (0.4411,0.4034) (0.4436,0.4056) (0.4461,0.4082) (0.4486,0.4107) (0.4511,0.4131) (0.4536,0.4154) (0.4561,0.4181) (0.4586,0.4205) (0.4612,0.4228) (0.4637,0.4250) (0.4662,0.4274) (0.4687,0.4301) (0.4712,0.4325) (0.4737,0.4350) (0.4762,0.4373) (0.4787,0.4397) (0.4812,0.4422) (0.4837,0.4445) (0.4862,0.4470) (0.4887,0.4493) (0.4912,0.4515) (0.4937,0.4538) (0.4962,0.4563) (0.4987,0.4587) (0.5013,0.4612) (0.5038,0.4634) (0.5063,0.4656) (0.5088,0.4681) (0.5113,0.4704) (0.5138,0.4728) (0.5163,0.4752) (0.5188,0.4776) (0.5213,0.4799) (0.5238,0.4824) (0.5263,0.4850) (0.5288,0.4873) (0.5313,0.4898) (0.5338,0.4921) (0.5363,0.4945) (0.5388,0.4968) (0.5414,0.4992) (0.5439,0.5016) (0.5464,0.5040) (0.5489,0.5062) (0.5514,0.5085) (0.5539,0.5108) (0.5564,0.5131) (0.5589,0.5154) (0.5614,0.5176) (0.5639,0.5202) (0.5664,0.5226) (0.5689,0.5248) (0.5714,0.5271) (0.5739,0.5294) (0.5764,0.5316) (0.5789,0.5340) (0.5815,0.5364) (0.5840,0.5386) (0.5865,0.5411) (0.5890,0.5434) (0.5915,0.5456) (0.5940,0.5482) (0.5965,0.5505) (0.5990,0.5528) (0.6015,0.5554) (0.6040,0.5577) (0.6065,0.5602) (0.6090,0.5625) (0.6115,0.5650) (0.6140,0.5674) (0.6165,0.5697) (0.6190,0.5722) (0.6216,0.5746) (0.6241,0.5774) (0.6266,0.5799) (0.6291,0.5822) (0.6316,0.5845) (0.6341,0.5870) (0.6366,0.5895) (0.6391,0.5919) (0.6416,0.5941) (0.6441,0.5964) (0.6466,0.5987) (0.6491,0.6013) (0.6516,0.6035) (0.6541,0.6059) (0.6566,0.6085) (0.6591,0.6113) (0.6617,0.6135) (0.6642,0.6158) (0.6667,0.6186) (0.6692,0.6207) (0.6717,0.6230) (0.6742,0.6252) (0.6767,0.6276) (0.6792,0.6297) (0.6817,0.6321) (0.6842,0.6345) (0.6867,0.6367) (0.6892,0.6391) (0.6917,0.6416) (0.6942,0.6440) (0.6967,0.6463) (0.6992,0.6487) (0.7018,0.6511) (0.7043,0.6532) (0.7068,0.6554) (0.7093,0.6580) (0.7118,0.6604) (0.7143,0.6628) (0.7168,0.6649) (0.7193,0.6676) (0.7218,0.6700) (0.7243,0.6722) (0.7268,0.6745) (0.7293,0.6769) (0.7318,0.6792) (0.7343,0.6817) (0.7368,0.6838) (0.7393,0.6860) (0.7419,0.6884) (0.7444,0.6905) (0.7469,0.6929) (0.7494,0.6952) (0.7519,0.6979) (0.7544,0.7002) (0.7569,0.7028) (0.7594,0.7053) (0.7619,0.7077) (0.7644,0.7100) (0.7669,0.7123) (0.7694,0.7149) (0.7719,0.7174) (0.7744,0.7199) (0.7769,0.7224) (0.7794,0.7247) (0.7820,0.7271) (0.7845,0.7295) (0.7870,0.7320) (0.7895,0.7342) (0.7920,0.7366) (0.7945,0.7388) (0.7970,0.7411) (0.7995,0.7435) (0.8020,0.7458) (0.8045,0.7480) (0.8070,0.7505) (0.8095,0.7528) (0.8120,0.7553) (0.8145,0.7576) (0.8170,0.7601) (0.8195,0.7625) (0.8221,0.7646) (0.8246,0.7667) (0.8271,0.7692) (0.8296,0.7714) (0.8321,0.7739) (0.8346,0.7763) (0.8371,0.7787) (0.8396,0.7811) (0.8421,0.7833) (0.8446,0.7857) (0.8471,0.7884) (0.8496,0.7905) (0.8521,0.7929) (0.8546,0.7954) (0.8571,0.7978) (0.8596,0.8003) (0.8622,0.8028) (0.8647,0.8054) (0.8672,0.8079) (0.8697,0.8102) (0.8722,0.8125) (0.8747,0.8147) (0.8772,0.8170) (0.8797,0.8194) (0.8822,0.8219) (0.8847,0.8243) (0.8872,0.8270) (0.8897,0.8294) (0.8922,0.8316) (0.8947,0.8339) (0.8972,0.8363) (0.8997,0.8388) (0.9023,0.8409) (0.9048,0.8433) (0.9073,0.8458) (0.9098,0.8483) (0.9123,0.8508) (0.9148,0.8532) (0.9173,0.8557) (0.9198,0.8580) (0.9223,0.8603) (0.9248,0.8626) (0.9273,0.8650) (0.9298,0.8673) (0.9323,0.8695) (0.9348,0.8722) (0.9373,0.8745) (0.9398,0.8769) (0.9424,0.8793) (0.9449,0.8817) (0.9474,0.8840) (0.9499,0.8865) (0.9524,0.8889) (0.9549,0.8914) (0.9574,0.8937) (0.9599,0.8961) (0.9624,0.8986) (0.9649,0.9009) (0.9674,0.9036) (0.9699,0.9060) (0.9724,0.9083) (0.9749,0.9107) (0.9774,0.9130) (0.9799,0.9154) (0.9825,0.9180) (0.9850,0.9203) (0.9875,0.9226) (0.9900,0.9251) (0.9925,0.9275) (0.9950,0.9299) (0.9975,0.9323) (1.0000,0.9349)};


==> figures/autogenerated/jdt-slide-05x05-bare-content.tex <==
% AUTO-GENERATED FILE -- do not edit by hand.
% Created by notebooks/figures/08_jdt_slide_figures.ipynb
% (orchestrated by libraries/visualization/jdt_slide.py).
% To regenerate, run that notebook.

\node[visible node] at (0.5,0.5) {$1$}; 
\node[visible node] at (0.5,1.5) {$3$}; 
\node[visible node] at (0.5,2.5) {$5$}; 
\node[visible node] at (0.5,3.5) {$6$}; 
\node[visible node] at (0.5,4.5) {$10$}; 
\node[visible node] at (1.5,0.5) {$2$}; 
\node[visible node] at (1.5,1.5) {$4$}; 
\node[visible node] at (1.5,2.5) {$8$}; 
\node[visible node] at (1.5,3.5) {$16$}; 
\node[visible node] at (1.5,4.5) {$28$}; 
\node[visible node] at (2.5,0.5) {$7$}; 
\node[visible node] at (2.5,1.5) {$11$}; 
\node[visible node] at (2.5,2.5) {$14$}; 
\node[visible node] at (2.5,3.5) {$25$}; 
\node[visible node] at (2.5,4.5) {$36$}; 
\node[visible node] at (3.5,0.5) {$9$}; 
\node[visible node] at (3.5,1.5) {$12$}; 
\node[visible node] at (3.5,2.5) {$17$}; 
\node[visible node] at (3.5,3.5) {$33$}; 
\node[visible node] at (3.5,4.5) {$49$}; 
\node[visible node] at (4.5,0.5) {$13$}; 
\node[visible node] at (4.5,1.5) {$21$}; 
\node[visible node] at (4.5,2.5) {$40$}; 
\node[visible node] at (4.5,3.5) {$42$}; 
\node[visible node] at (4.5,4.5) {$52$}; 


==> figures/autogenerated/jdt-slide-09x09-after-annotations.tex <==
% Boundary annotations ($z_i$ bubbles) for a jeu-de-taquin-slide figure.
% Source: notebooks/figures/08_jdt_slide_figures.ipynb in trees-SageMath
% (orchestrated by SageMath/libraries/visualization/jdt_slide.py), but the
% bubble positions MAY HAVE BEEN ADJUSTED BY HAND.  The generator does NOT
% overwrite this file when it already exists, so manual edits are preserved;
% delete the file first if you want it regenerated from scratch.

\node[circle, draw=black, fill=vertex-z2] at (3.5,10.0) {$z_{2}$};
\node[circle, draw=black, fill=vertex-z3] at (10.0,1.5) {$z_{3}$};
\node[circle, draw=black, fill=vertex-z5] at (10.0,4.5) {$z_{5}$};
\node[circle, draw=black, fill=vertex-z13] at (7.5,10.0) {\textcolor{white}{$z_{13}$}};
\node[circle, draw=black, fill=vertex-z14] at (10.0,6.5) {$z_{14}$};


==> figures/autogenerated/jdt-slide-09x09-after-content.tex <==
% AUTO-GENERATED FILE -- do not edit by hand.
% Source: notebooks/figures/08_jdt_slide_figures.ipynb in trees-SageMath
% (orchestrated by SageMath/libraries/visualization/jdt_slide.py).
% To regenerate, run that notebook.

\fill[competition interface,vertex-z3] (9.00,0.00) -- (8.00,0.00) -- (7.00,0.00) -- (6.00,0.00) -- (5.00,0.00) -- (4.00,0.00) -- (3.00,0.00) -- (2.00,0.00) -- (1.00,0.00) -- (1.00,1.00) -- (1.00,2.00) -- (2.00,2.00) -- (3.00,2.00) -- (4.00,2.00) -- (5.00,2.00) -- (6.00,2.00) -- (7.00,2.00) -- (8.00,2.00) -- (8.00,3.00) -- (9.00,3.00); 
\fill[competition interface,vertex-z5] (9.00,3.00) -- (8.00,3.00) -- (8.00,2.00) -- (7.00,2.00) -- (6.00,2.00) -- (5.00,2.00) -- (4.00,2.00) -- (3.00,2.00) -- (3.00,3.00) -- (4.00,3.00) -- (4.00,4.00) -- (5.00,4.00) -- (5.00,5.00) -- (6.00,5.00) -- (7.00,5.00) -- (8.00,5.00) -- (9.00,5.00); 
\fill[competition interface,vertex-z14] (9.00,5.00) -- (8.00,5.00) -- (7.00,5.00) -- (6.00,5.00) -- (6.00,6.00) -- (7.00,6.00) -- (7.00,7.00) -- (8.00,7.00) -- (8.00,8.00) -- (9.00,8.00); 
\fill[competition interface,vertex-z13] (9.00,8.00) -- (8.00,8.00) -- (8.00,7.00) -- (7.00,7.00) -- (7.00,6.00) -- (6.00,6.00) -- (6.00,7.00) -- (6.00,8.00) -- (6.00,9.00) -- (9.00,9.00); 
\fill[competition interface,vertex-z2] (6.00,9.00) -- (6.00,8.00) -- (6.00,7.00) -- (6.00,6.00) -- (6.00,5.00) -- (5.00,5.00) -- (5.00,4.00) -- (4.00,4.00) -- (4.00,3.00) -- (3.00,3.00) -- (3.00,2.00) -- (2.00,2.00) -- (1.00,2.00) -- (1.00,1.00) -- (1.00,0.00) -- (0.00,0.00) -- (0.00,1.00) -- (0.00,2.00) -- (0.00,3.00) -- (0.00,4.00) -- (0.00,5.00) -- (0.00,6.00) -- (0.00,7.00) -- (0.00,8.00) -- (0.00,9.00); 
\gridcommand
\draw[jdt path] (0.5,0.5) -- (1.5,0.5) -- (1.5,1.5) -- (1.5,2.5) -- (2.5,2.5) -- (3.5,2.5) -- (3.5,3.5) -- (4.5,3.5) -- (4.5,4.5) -- (5.5,4.5) -- (5.5,5.5) -- (6.5,5.5) -- (7.5,5.5) -- (8.5,5.5) -- (9.5,5.5);
\node[invisible node] (node-0-0) at (0.5,0.5) {}; 
\node[invisible node] (node-0-1) at (0.5,1.5) {}; 
\node[invisible node] (node-0-2) at (0.5,2.5) {}; 
\node[invisible node] (node-0-3) at (0.5,3.5) {}; 
\node[invisible node] (node-0-4) at (0.5,4.5) {}; 
\node[invisible node] (node-0-5) at (0.5,5.5) {}; 
\node[invisible node] (node-0-6) at (0.5,6.5) {}; 
\node[invisible node] (node-0-7) at (0.5,7.5) {}; 
\node[invisible node] (node-0-8) at (0.5,8.5) {}; 
\node[invisible node] (node-0-9) at (0.5,9.5) {}; 
\node[invisible node] (node-1-0) at (1.5,0.5) {}; 
\node[invisible node] (node-1-1) at (1.5,1.5) {}; 
\node[invisible node] (node-1-2) at (1.5,2.5) {}; 
\node[invisible node] (node-1-3) at (1.5,3.5) {}; 
\node[invisible node] (node-1-4) at (1.5,4.5) {}; 
\node[invisible node] (node-1-5) at (1.5,5.5) {}; 
\node[invisible node] (node-1-6) at (1.5,6.5) {}; 
\node[invisible node] (node-1-7) at (1.5,7.5) {}; 
\node[invisible node] (node-1-8) at (1.5,8.5) {}; 
\node[invisible node] (node-1-9) at (1.5,9.5) {}; 
\node[invisible node] (node-2-0) at (2.5,0.5) {}; 
\node[invisible node] (node-2-1) at (2.5,1.5) {}; 
\node[invisible node] (node-2-2) at (2.5,2.5) {}; 
\node[invisible node] (node-2-3) at (2.5,3.5) {}; 
\node[invisible node] (node-2-4) at (2.5,4.5) {}; 
\node[invisible node] (node-2-5) at (2.5,5.5) {}; 
\node[invisible node] (node-2-6) at (2.5,6.5) {}; 
\node[invisible node] (node-2-7) at (2.5,7.5) {}; 
\node[invisible node] (node-2-8) at (2.5,8.5) {}; 
\node[invisible node] (node-2-9) at (2.5,9.5) {}; 
\node[invisible node] (node-3-0) at (3.5,0.5) {}; 
\node[invisible node] (node-3-1) at (3.5,1.5) {}; 
\node[invisible node] (node-3-2) at (3.5,2.5) {}; 
\node[invisible node] (node-3-3) at (3.5,3.5) {}; 
\node[invisible node] (node-3-4) at (3.5,4.5) {}; 
\node[invisible node] (node-3-5) at (3.5,5.5) {}; 
\node[invisible node] (node-3-6) at (3.5,6.5) {}; 
\node[invisible node] (node-3-7) at (3.5,7.5) {}; 
\node[invisible node] (node-3-8) at (3.5,8.5) {}; 
\node[invisible node] (node-3-9) at (3.5,9.5) {}; 
\node[invisible node] (node-4-0) at (4.5,0.5) {}; 
\node[invisible node] (node-4-1) at (4.5,1.5) {}; 
\node[invisible node] (node-4-2) at (4.5,2.5) {}; 
\node[invisible node] (node-4-3) at (4.5,3.5) {}; 
\node[invisible node] (node-4-4) at (4.5,4.5) {}; 
\node[invisible node] (node-4-5) at (4.5,5.5) {}; 
\node[invisible node] (node-4-6) at (4.5,6.5) {}; 
\node[invisible node] (node-4-7) at (4.5,7.5) {}; 
\node[invisible node] (node-4-8) at (4.5,8.5) {}; 
\node[invisible node] (node-4-9) at (4.5,9.5) {}; 
\node[invisible node] (node-5-0) at (5.5,0.5) {}; 
\node[invisible node] (node-5-1) at (5.5,1.5) {}; 
\node[invisible node] (node-5-2) at (5.5,2.5) {}; 
\node[invisible node] (node-5-3) at (5.5,3.5) {}; 
\node[invisible node] (node-5-4) at (5.5,4.5) {}; 
\node[invisible node] (node-5-5) at (5.5,5.5) {}; 
\node[invisible node] (node-5-6) at (5.5,6.5) {}; 
\node[invisible node] (node-5-7) at (5.5,7.5) {}; 
\node[invisible node] (node-5-8) at (5.5,8.5) {}; 
\node[invisible node] (node-5-9) at (5.5,9.5) {}; 
\node[invisible node] (node-6-0) at (6.5,0.5) {}; 
\node[invisible node] (node-6-1) at (6.5,1.5) {}; 
\node[invisible node] (node-6-2) at (6.5,2.5) {}; 
\node[invisible node] (node-6-3) at (6.5,3.5) {}; 
\node[invisible node] (node-6-4) at (6.5,4.5) {}; 
\node[invisible node] (node-6-5) at (6.5,5.5) {}; 
\node[invisible node] (node-6-6) at (6.5,6.5) {}; 
\node[invisible node] (node-6-7) at (6.5,7.5) {}; 
\node[invisible node] (node-6-8) at (6.5,8.5) {}; 
\node[invisible node] (node-6-9) at (6.5,9.5) {}; 
\node[invisible node] (node-7-0) at (7.5,0.5) {}; 
\node[invisible node] (node-7-1) at (7.5,1.5) {}; 
\node[invisible node] (node-7-2) at (7.5,2.5) {}; 
\node[invisible node] (node-7-3) at (7.5,3.5) {}; 
\node[invisible node] (node-7-4) at (7.5,4.5) {}; 
\node[invisible node] (node-7-5) at (7.5,5.5) {}; 
\node[invisible node] (node-7-6) at (7.5,6.5) {}; 
\node[invisible node] (node-7-7) at (7.5,7.5) {}; 
\node[invisible node] (node-7-8) at (7.5,8.5) {}; 
\node[invisible node] (node-7-9) at (7.5,9.5) {}; 
\node[invisible node] (node-8-0) at (8.5,0.5) {}; 
\node[invisible node] (node-8-1) at (8.5,1.5) {}; 
\node[invisible node] (node-8-2) at (8.5,2.5) {}; 
\node[invisible node] (node-8-3) at (8.5,3.5) {}; 
\node[invisible node] (node-8-4) at (8.5,4.5) {}; 
\node[invisible node] (node-8-5) at (8.5,5.5) {}; 
\node[invisible node] (node-8-6) at (8.5,6.5) {}; 
\node[invisible node] (node-8-7) at (8.5,7.5) {}; 
\node[invisible node] (node-8-8) at (8.5,8.5) {}; 
\node[invisible node] (node-8-9) at (8.5,9.5) {}; 
\node[invisible node] (node-9-0) at (9.5,0.5) {}; 
\node[invisible node] (node-9-1) at (9.5,1.5) {}; 
\node[invisible node] (node-9-2) at (9.5,2.5) {}; 
\node[invisible node] (node-9-3) at (9.5,3.5) {}; 
\node[invisible node] (node-9-4) at (9.5,4.5) {}; 
\node[invisible node] (node-9-5) at (9.5,5.5) {}; 
\node[invisible node] (node-9-6) at (9.5,6.5) {}; 
\node[invisible node] (node-9-7) at (9.5,7.5) {}; 
\node[invisible node] (node-9-8) at (9.5,8.5) {}; 
\node[invisible node] (node-9-9) at (9.5,9.5) {}; 
\node[visible node] at (0.5,0.5) {$2$}; 
\node[visible node] at (0.5,1.5) {$3$}; 
\node[visible node] at (0.5,2.5) {$5$}; 
\node[visible node] at (0.5,3.5) {$6$}; 
\node[visible node] at (0.5,4.5) {$10$}; 
\node[visible node] at (0.5,5.5) {$20$}; 
\node[visible node] at (0.5,6.5) {$22$}; 
\node[visible node] at (0.5,7.5) {$26$}; 
\node[visible node] at (0.5,8.5) {$32$}; 
\node[visible node] at (1.5,0.5) {$4$}; 
\node[visible node] at (1.5,1.5) {$8$}; 
\node[visible node] at (1.5,2.5) {$14$}; 
\node[visible node] at (1.5,3.5) {$16$}; 
\node[visible node] at (1.5,4.5) {$28$}; 
\node[visible node] at (1.5,5.5) {$31$}; 
\node[visible node] at (1.5,6.5) {$38$}; 
\node[visible node] at (1.5,7.5) {$46$}; 
\node[visible node] at (1.5,8.5) {$47$}; 
\node[visible node] at (2.5,0.5) {$7$}; 
\node[visible node] at (2.5,1.5) {$11$}; 
\node[visible node] at (2.5,2.5) {$17$}; 
\node[visible node] at (2.5,3.5) {$25$}; 
\node[visible node] at (2.5,4.5) {$36$}; 
\node[visible node] at (2.5,5.5) {$39$}; 
\node[visible node] at (2.5,6.5) {$45$}; 
\node[visible node] at (2.5,7.5) {$50$}; 
\node[visible node] at (2.5,8.5) {$53$}; 
\node[visible node] at (3.5,0.5) {$9$}; 
\node[visible node] at (3.5,1.5) {$12$}; 
\node[visible node] at (3.5,2.5) {$33$}; 
\node[visible node] at (3.5,3.5) {$42$}; 
\node[visible node] at (3.5,4.5) {$49$}; 
\node[visible node] at (3.5,5.5) {$66$}; 
\node[visible node] at (3.5,6.5) {$70$}; 
\node[visible node] at (3.5,7.5) {$77$}; 
\node[visible node] at (3.5,8.5) {$103$}; 
\node[visible node] at (4.5,0.5) {$13$}; 
\node[visible node] at (4.5,1.5) {$21$}; 
\node[visible node] at (4.5,2.5) {$40$}; 
\node[visible node] at (4.5,3.5) {$52$}; 
\node[visible node] at (4.5,4.5) {$61$}; 
\node[visible node] at (4.5,5.5) {$68$}; 
\node[visible node] at (4.5,6.5) {$88$}; 
\node[visible node] at (4.5,7.5) {$95$}; 
\node[visible node] at (4.5,8.5) {$106$}; 
\node[visible node] at (5.5,0.5) {$15$}; 
\node[visible node] at (5.5,1.5) {$24$}; 
\node[visible node] at (5.5,2.5) {$41$}; 
\node[visible node] at (5.5,3.5) {$57$}; 
\node[visible node] at (5.5,4.5) {$72$}; 
\node[visible node] at (5.5,5.5) {$76$}; 
\node[visible node] at (5.5,6.5) {$92$}; 
\node[visible node] at (5.5,7.5) {$105$}; 
\node[visible node] at (5.5,8.5) {$110$}; 
\node[visible node] at (6.5,0.5) {$18$}; 
\node[visible node] at (6.5,1.5) {$29$}; 
\node[visible node] at (6.5,2.5) {$44$}; 
\node[visible node] at (6.5,3.5) {$59$}; 
\node[visible node] at (6.5,4.5) {$74$}; 
\node[visible node] at (6.5,5.5) {$100$}; 
\node[visible node] at (6.5,6.5) {$116$}; 
\node[visible node] at (6.5,7.5) {$126$}; 
\node[visible node] at (6.5,8.5) {$143$}; 
\node[visible node] at (7.5,0.5) {$19$}; 
\node[visible node] at (7.5,1.5) {$30$}; 
\node[visible node] at (7.5,2.5) {$51$}; 
\node[visible node] at (7.5,3.5) {$62$}; 
\node[visible node] at (7.5,4.5) {$85$}; 
\node[visible node] at (7.5,5.5) {$104$}; 
\node[visible node] at (7.5,6.5) {$133$}; 
\node[visible node] at (7.5,7.5) {$149$}; 
\node[visible node] at (7.5,8.5) {$155$}; 
\node[visible node] at (8.5,0.5) {$23$}; 
\node[visible node] at (8.5,1.5) {$48$}; 
\node[visible node] at (8.5,2.5) {$69$}; 
\node[visible node] at (8.5,3.5) {$82$}; 
\node[visible node] at (8.5,4.5) {$93$}; 
\node[visible node] at (8.5,5.5) {$124$}; 
\node[visible node] at (8.5,6.5) {$144$}; 
\node[visible node] at (8.5,7.5) {$166$}; 
\node[visible node] at (8.5,8.5) {$225$}; 
\draw[edge changed] (node-0-0) -- (node-0-1);
\draw[edge changed] (node-0-1) -- (node-0-2);
\draw[edge] (node-0-2) -- (node-0-3);
\draw[edge] (node-0-3) -- (node-0-4);
\draw[edge] (node-0-4) -- (node-0-5);
\draw[edge] (node-0-5) -- (node-0-6);
\draw[edge] (node-0-6) -- (node-0-7);
\draw[edge] (node-0-7) -- (node-0-8);
\draw[edge] (node-0-8) -- (node-0-9);
\draw[edge changed] (node-1-0) -- (node-2-0);
\draw[edge changed] (node-1-1) -- (node-2-1);
\draw[edge changed] (node-1-2) -- (node-1-3);
\draw[edge] (node-1-3) -- (node-2-3);
\draw[edge] (node-1-4) -- (node-1-5);
\draw[edge] (node-1-5) -- (node-1-6);
\draw[edge] (node-1-6) -- (node-2-6);
\draw[edge] (node-1-7) -- (node-1-8);
\draw[edge] (node-1-8) -- (node-2-8);
\draw[edge] (node-2-0) -- (node-3-0);
\draw[edge] (node-2-1) -- (node-3-1);
\draw[edge changed] (node-2-2) -- (node-2-3);
\draw[edge changed] (node-2-3) -- (node-2-4);
\draw[edge] (node-2-4) -- (node-2-5);
\draw[edge] (node-2-5) -- (node-2-6);
\draw[edge] (node-2-6) -- (node-2-7);
\draw[edge] (node-2-7) -- (node-2-8);
\draw[edge] (node-2-8) -- (node-2-9);
\draw[edge] (node-3-0) -- (node-3-1);
\draw[edge changed] (node-3-1) -- (node-4-1);
\draw[edge changed] (node-3-2) -- (node-4-2);
\draw[edge changed] (node-3-3) -- (node-3-4);
\draw[edge] (node-3-4) -- (node-4-4);
\draw[edge] (node-3-5) -- (node-4-5);
\draw[edge] (node-3-6) -- (node-3-7);
\draw[edge] (node-3-7) -- (node-4-7);
\draw[edge] (node-3-8) -- (node-4-8);
\draw[edge] (node-4-0) -- (node-5-0);
\draw[edge] (node-4-1) -- (node-5-1);
\draw[edge] (node-4-2) -- (node-5-2);
\draw[edge changed] (node-4-3) -- (node-5-3);
\draw[edge changed] (node-4-4) -- (node-4-5);
\draw[edge] (node-4-5) -- (node-5-5);
\draw[edge] (node-4-6) -- (node-5-6);
\draw[edge] (node-4-7) -- (node-5-7);
\draw[edge] (node-4-8) -- (node-5-8);
\draw[edge] (node-5-0) -- (node-6-0);
\draw[edge] (node-5-1) -- (node-6-1);
\draw[edge] (node-5-2) -- (node-6-2);
\draw[edge] (node-5-3) -- (node-6-3);
\draw[edge changed] (node-5-4) -- (node-6-4);
\draw[edge changed] (node-5-5) -- (node-5-6);
\draw[edge] (node-5-6) -- (node-5-7);
\draw[edge] (node-5-7) -- (node-5-8);
\draw[edge] (node-5-8) -- (node-5-9);
\draw[edge] (node-6-0) -- (node-7-0);
\draw[edge] (node-6-1) -- (node-7-1);
\draw[edge] (node-6-2) -- (node-7-2);
\draw[edge] (node-6-3) -- (node-7-3);
\draw[edge changed] (node-6-4) -- (node-7-4);
\draw[edge] (node-6-5) -- (node-7-5);
\draw[edge] (node-6-6) -- (node-6-7);
\draw[edge] (node-6-7) -- (node-6-8);
\draw[edge] (node-6-8) -- (node-7-8);
\draw[edge] (node-7-0) -- (node-8-0);
\draw[edge] (node-7-1) -- (node-8-1);
\draw[edge] (node-7-2) -- (node-7-3);
\draw[edge] (node-7-3) -- (node-8-3);
\draw[edge] (node-7-4) -- (node-8-4);
\draw[edge] (node-7-5) -- (node-8-5);
\draw[edge] (node-7-6) -- (node-8-6);
\draw[edge] (node-7-7) -- (node-7-8);
\draw[edge] (node-7-8) -- (node-7-9);
\draw[edge] (node-8-0) -- (node-9-0);
\draw[edge] (node-8-1) -- (node-9-1);
\draw[edge] (node-8-2) -- (node-9-2);
\draw[edge] (node-8-3) -- (node-9-3);
\draw[edge changed] (node-8-4) -- (node-9-4);
\draw[edge] (node-8-5) -- (node-9-5);
\draw[edge] (node-8-6) -- (node-9-6);
\draw[edge] (node-8-7) -- (node-9-7);
\draw[edge] (node-8-8) -- (node-8-9);
\node[highlight box] at (0.5,1.5) {};
\node[highlight box] at (2.5,3.5) {};
\node[highlight box] at (3.5,1.5) {};
\node[highlight box] at (5.5,5.5) {};


==> figures/autogenerated/jdt-slide-09x09-before-annotations.tex <==
% Boundary annotations ($z_i$ bubbles) for a jeu-de-taquin-slide figure.
% Source: notebooks/figures/08_jdt_slide_figures.ipynb in trees-SageMath
% (orchestrated by SageMath/libraries/visualization/jdt_slide.py), but the
% bubble positions MAY HAVE BEEN ADJUSTED BY HAND.  The generator does NOT
% overwrite this file when it already exists, so manual edits are preserved;
% delete the file first if you want it regenerated from scratch.

\node[circle, draw=black, fill=vertex-z1] at (10.0,4.5) {$z_{1}$};
\node[circle, draw=black, fill=vertex-z2] at (3.5,10.0) {$z_{2}$};
\node[circle, draw=black, fill=vertex-z3] at (10.0,1.5) {$z_{3}$};
\node[circle, draw=black, fill=vertex-z13] at (7.5,10.0) {\textcolor{white}{$z_{13}$}};
\node[circle, draw=black, fill=vertex-z14] at (10.0,6.5) {$z_{14}$};


==> figures/autogenerated/jdt-slide-09x09-before-content.tex <==
% AUTO-GENERATED FILE -- do not edit by hand.
% Source: notebooks/figures/08_jdt_slide_figures.ipynb in trees-SageMath
% (orchestrated by SageMath/libraries/visualization/jdt_slide.py).
% To regenerate, run that notebook.

\fill[competition interface,vertex-z3] (9.00,0.00) -- (8.00,0.00) -- (7.00,0.00) -- (6.00,0.00) -- (5.00,0.00) -- (4.00,0.00) -- (4.00,1.00) -- (4.00,2.00) -- (5.00,2.00) -- (6.00,2.00) -- (7.00,2.00) -- (8.00,2.00) -- (8.00,3.00) -- (9.00,3.00); 
\fill[competition interface,vertex-z1] (9.00,3.00) -- (8.00,3.00) -- (8.00,2.00) -- (7.00,2.00) -- (6.00,2.00) -- (5.00,2.00) -- (4.00,2.00) -- (4.00,1.00) -- (4.00,0.00) -- (3.00,0.00) -- (2.00,0.00) -- (1.00,0.00) -- (0.00,0.00) -- (0.00,1.00) -- (0.00,2.00) -- (1.00,2.00) -- (1.00,3.00) -- (1.00,4.00) -- (2.00,4.00) -- (3.00,4.00) -- (3.00,5.00) -- (3.00,6.00) -- (4.00,6.00) -- (5.00,6.00) -- (6.00,6.00) -- (7.00,6.00) -- (8.00,6.00) -- (9.00,6.00); 
\fill[competition interface,vertex-z14] (9.00,6.00) -- (8.00,6.00) -- (7.00,6.00) -- (7.00,7.00) -- (8.00,7.00) -- (8.00,8.00) -- (9.00,8.00); 
\fill[competition interface,vertex-z13] (9.00,8.00) -- (8.00,8.00) -- (8.00,7.00) -- (7.00,7.00) -- (7.00,6.00) -- (6.00,6.00) -- (6.00,7.00) -- (6.00,8.00) -- (6.00,9.00) -- (9.00,9.00); 
\fill[competition interface,vertex-z2] (6.00,9.00) -- (6.00,8.00) -- (6.00,7.00) -- (6.00,6.00) -- (5.00,6.00) -- (4.00,6.00) -- (3.00,6.00) -- (3.00,5.00) -- (3.00,4.00) -- (2.00,4.00) -- (1.00,4.00) -- (1.00,3.00) -- (1.00,2.00) -- (0.00,2.00) -- (0.00,3.00) -- (0.00,4.00) -- (0.00,5.00) -- (0.00,6.00) -- (0.00,7.00) -- (0.00,8.00) -- (0.00,9.00); 
\gridcommand
\draw[jdt path] (0.5,0.5) -- (1.5,0.5) -- (1.5,1.5) -- (1.5,2.5) -- (2.5,2.5) -- (3.5,2.5) -- (3.5,3.5) -- (4.5,3.5) -- (4.5,4.5) -- (5.5,4.5) -- (5.5,5.5) -- (6.5,5.5) -- (7.5,5.5) -- (8.5,5.5) -- (9.5,5.5);
\node[invisible node] (node-0-0) at (0.5,0.5) {}; 
\node[invisible node] (node-0-1) at (0.5,1.5) {}; 
\node[invisible node] (node-0-2) at (0.5,2.5) {}; 
\node[invisible node] (node-0-3) at (0.5,3.5) {}; 
\node[invisible node] (node-0-4) at (0.5,4.5) {}; 
\node[invisible node] (node-0-5) at (0.5,5.5) {}; 
\node[invisible node] (node-0-6) at (0.5,6.5) {}; 
\node[invisible node] (node-0-7) at (0.5,7.5) {}; 
\node[invisible node] (node-0-8) at (0.5,8.5) {}; 
\node[invisible node] (node-0-9) at (0.5,9.5) {}; 
\node[invisible node] (node-1-0) at (1.5,0.5) {}; 
\node[invisible node] (node-1-1) at (1.5,1.5) {}; 
\node[invisible node] (node-1-2) at (1.5,2.5) {}; 
\node[invisible node] (node-1-3) at (1.5,3.5) {}; 
\node[invisible node] (node-1-4) at (1.5,4.5) {}; 
\node[invisible node] (node-1-5) at (1.5,5.5) {}; 
\node[invisible node] (node-1-6) at (1.5,6.5) {}; 
\node[invisible node] (node-1-7) at (1.5,7.5) {}; 
\node[invisible node] (node-1-8) at (1.5,8.5) {}; 
\node[invisible node] (node-1-9) at (1.5,9.5) {}; 
\node[invisible node] (node-2-0) at (2.5,0.5) {}; 
\node[invisible node] (node-2-1) at (2.5,1.5) {}; 
\node[invisible node] (node-2-2) at (2.5,2.5) {}; 
\node[invisible node] (node-2-3) at (2.5,3.5) {}; 
\node[invisible node] (node-2-4) at (2.5,4.5) {}; 
\node[invisible node] (node-2-5) at (2.5,5.5) {}; 
\node[invisible node] (node-2-6) at (2.5,6.5) {}; 
\node[invisible node] (node-2-7) at (2.5,7.5) {}; 
\node[invisible node] (node-2-8) at (2.5,8.5) {}; 
\node[invisible node] (node-2-9) at (2.5,9.5) {}; 
\node[invisible node] (node-3-0) at (3.5,0.5) {}; 
\node[invisible node] (node-3-1) at (3.5,1.5) {}; 
\node[invisible node] (node-3-2) at (3.5,2.5) {}; 
\node[invisible node] (node-3-3) at (3.5,3.5) {}; 
\node[invisible node] (node-3-4) at (3.5,4.5) {}; 
\node[invisible node] (node-3-5) at (3.5,5.5) {}; 
\node[invisible node] (node-3-6) at (3.5,6.5) {}; 
\node[invisible node] (node-3-7) at (3.5,7.5) {}; 
\node[invisible node] (node-3-8) at (3.5,8.5) {}; 
\node[invisible node] (node-3-9) at (3.5,9.5) {}; 
\node[invisible node] (node-4-0) at (4.5,0.5) {}; 
\node[invisible node] (node-4-1) at (4.5,1.5) {}; 
\node[invisible node] (node-4-2) at (4.5,2.5) {}; 
\node[invisible node] (node-4-3) at (4.5,3.5) {}; 
\node[invisible node] (node-4-4) at (4.5,4.5) {}; 
\node[invisible node] (node-4-5) at (4.5,5.5) {}; 
\node[invisible node] (node-4-6) at (4.5,6.5) {}; 
\node[invisible node] (node-4-7) at (4.5,7.5) {}; 
\node[invisible node] (node-4-8) at (4.5,8.5) {}; 
\node[invisible node] (node-4-9) at (4.5,9.5) {}; 
\node[invisible node] (node-5-0) at (5.5,0.5) {}; 
\node[invisible node] (node-5-1) at (5.5,1.5) {}; 
\node[invisible node] (node-5-2) at (5.5,2.5) {}; 
\node[invisible node] (node-5-3) at (5.5,3.5) {}; 
\node[invisible node] (node-5-4) at (5.5,4.5) {}; 
\node[invisible node] (node-5-5) at (5.5,5.5) {}; 
\node[invisible node] (node-5-6) at (5.5,6.5) {}; 
\node[invisible node] (node-5-7) at (5.5,7.5) {}; 
\node[invisible node] (node-5-8) at (5.5,8.5) {}; 
\node[invisible node] (node-5-9) at (5.5,9.5) {}; 
\node[invisible node] (node-6-0) at (6.5,0.5) {}; 
\node[invisible node] (node-6-1) at (6.5,1.5) {}; 
\node[invisible node] (node-6-2) at (6.5,2.5) {}; 
\node[invisible node] (node-6-3) at (6.5,3.5) {}; 
\node[invisible node] (node-6-4) at (6.5,4.5) {}; 
\node[invisible node] (node-6-5) at (6.5,5.5) {}; 
\node[invisible node] (node-6-6) at (6.5,6.5) {}; 
\node[invisible node] (node-6-7) at (6.5,7.5) {}; 
\node[invisible node] (node-6-8) at (6.5,8.5) {}; 
\node[invisible node] (node-6-9) at (6.5,9.5) {}; 
\node[invisible node] (node-7-0) at (7.5,0.5) {}; 
\node[invisible node] (node-7-1) at (7.5,1.5) {}; 
\node[invisible node] (node-7-2) at (7.5,2.5) {}; 
\node[invisible node] (node-7-3) at (7.5,3.5) {}; 
\node[invisible node] (node-7-4) at (7.5,4.5) {}; 
\node[invisible node] (node-7-5) at (7.5,5.5) {}; 
\node[invisible node] (node-7-6) at (7.5,6.5) {}; 
\node[invisible node] (node-7-7) at (7.5,7.5) {}; 
\node[invisible node] (node-7-8) at (7.5,8.5) {}; 
\node[invisible node] (node-7-9) at (7.5,9.5) {}; 
\node[invisible node] (node-8-0) at (8.5,0.5) {}; 
\node[invisible node] (node-8-1) at (8.5,1.5) {}; 
\node[invisible node] (node-8-2) at (8.5,2.5) {}; 
\node[invisible node] (node-8-3) at (8.5,3.5) {}; 
\node[invisible node] (node-8-4) at (8.5,4.5) {}; 
\node[invisible node] (node-8-5) at (8.5,5.5) {}; 
\node[invisible node] (node-8-6) at (8.5,6.5) {}; 
\node[invisible node] (node-8-7) at (8.5,7.5) {}; 
\node[invisible node] (node-8-8) at (8.5,8.5) {}; 
\node[invisible node] (node-8-9) at (8.5,9.5) {}; 
\node[invisible node] (node-9-0) at (9.5,0.5) {}; 
\node[invisible node] (node-9-1) at (9.5,1.5) {}; 
\node[invisible node] (node-9-2) at (9.5,2.5) {}; 
\node[invisible node] (node-9-3) at (9.5,3.5) {}; 
\node[invisible node] (node-9-4) at (9.5,4.5) {}; 
\node[invisible node] (node-9-5) at (9.5,5.5) {}; 
\node[invisible node] (node-9-6) at (9.5,6.5) {}; 
\node[invisible node] (node-9-7) at (9.5,7.5) {}; 
\node[invisible node] (node-9-8) at (9.5,8.5) {}; 
\node[invisible node] (node-9-9) at (9.5,9.5) {}; 
\node[visible node] at (0.5,0.5) {$1$}; 
\node[visible node] at (0.5,1.5) {$3$}; 
\node[visible node] at (0.5,2.5) {$5$}; 
\node[visible node] at (0.5,3.5) {$6$}; 
\node[visible node] at (0.5,4.5) {$10$}; 
\node[visible node] at (0.5,5.5) {$20$}; 
\node[visible node] at (0.5,6.5) {$22$}; 
\node[visible node] at (0.5,7.5) {$26$}; 
\node[visible node] at (0.5,8.5) {$32$}; 
\node[visible node] at (1.5,0.5) {$2$}; 
\node[visible node] at (1.5,1.5) {$4$}; 
\node[visible node] at (1.5,2.5) {$8$}; 
\node[visible node] at (1.5,3.5) {$16$}; 
\node[visible node] at (1.5,4.5) {$28$}; 
\node[visible node] at (1.5,5.5) {$31$}; 
\node[visible node] at (1.5,6.5) {$38$}; 
\node[visible node] at (1.5,7.5) {$46$}; 
\node[visible node] at (1.5,8.5) {$47$}; 
\node[visible node] at (2.5,0.5) {$7$}; 
\node[visible node] at (2.5,1.5) {$11$}; 
\node[visible node] at (2.5,2.5) {$14$}; 
\node[visible node] at (2.5,3.5) {$25$}; 
\node[visible node] at (2.5,4.5) {$36$}; 
\node[visible node] at (2.5,5.5) {$39$}; 
\node[visible node] at (2.5,6.5) {$45$}; 
\node[visible node] at (2.5,7.5) {$50$}; 
\node[visible node] at (2.5,8.5) {$53$}; 
\node[visible node] at (3.5,0.5) {$9$}; 
\node[visible node] at (3.5,1.5) {$12$}; 
\node[visible node] at (3.5,2.5) {$17$}; 
\node[visible node] at (3.5,3.5) {$33$}; 
\node[visible node] at (3.5,4.5) {$49$}; 
\node[visible node] at (3.5,5.5) {$66$}; 
\node[visible node] at (3.5,6.5) {$70$}; 
\node[visible node] at (3.5,7.5) {$77$}; 
\node[visible node] at (3.5,8.5) {$103$}; 
\node[visible node] at (4.5,0.5) {$13$}; 
\node[visible node] at (4.5,1.5) {$21$}; 
\node[visible node] at (4.5,2.5) {$40$}; 
\node[visible node] at (4.5,3.5) {$42$}; 
\node[visible node] at (4.5,4.5) {$52$}; 
\node[visible node] at (4.5,5.5) {$68$}; 
\node[visible node] at (4.5,6.5) {$88$}; 
\node[visible node] at (4.5,7.5) {$95$}; 
\node[visible node] at (4.5,8.5) {$106$}; 
\node[visible node] at (5.5,0.5) {$15$}; 
\node[visible node] at (5.5,1.5) {$24$}; 
\node[visible node] at (5.5,2.5) {$41$}; 
\node[visible node] at (5.5,3.5) {$57$}; 
\node[visible node] at (5.5,4.5) {$61$}; 
\node[visible node] at (5.5,5.5) {$72$}; 
\node[visible node] at (5.5,6.5) {$92$}; 
\node[visible node] at (5.5,7.5) {$105$}; 
\node[visible node] at (5.5,8.5) {$110$}; 
\node[visible node] at (6.5,0.5) {$18$}; 
\node[visible node] at (6.5,1.5) {$29$}; 
\node[visible node] at (6.5,2.5) {$44$}; 
\node[visible node] at (6.5,3.5) {$59$}; 
\node[visible node] at (6.5,4.5) {$74$}; 
\node[visible node] at (6.5,5.5) {$76$}; 
\node[visible node] at (6.5,6.5) {$116$}; 
\node[visible node] at (6.5,7.5) {$126$}; 
\node[visible node] at (6.5,8.5) {$143$}; 
\node[visible node] at (7.5,0.5) {$19$}; 
\node[visible node] at (7.5,1.5) {$30$}; 
\node[visible node] at (7.5,2.5) {$51$}; 
\node[visible node] at (7.5,3.5) {$62$}; 
\node[visible node] at (7.5,4.5) {$85$}; 
\node[visible node] at (7.5,5.5) {$100$}; 
\node[visible node] at (7.5,6.5) {$133$}; 
\node[visible node] at (7.5,7.5) {$149$}; 
\node[visible node] at (7.5,8.5) {$155$}; 
\node[visible node] at (8.5,0.5) {$23$}; 
\node[visible node] at (8.5,1.5) {$48$}; 
\node[visible node] at (8.5,2.5) {$69$}; 
\node[visible node] at (8.5,3.5) {$82$}; 
\node[visible node] at (8.5,4.5) {$93$}; 
\node[visible node] at (8.5,5.5) {$104$}; 
\node[visible node] at (8.5,6.5) {$144$}; 
\node[visible node] at (8.5,7.5) {$166$}; 
\node[visible node] at (8.5,8.5) {$225$}; 
\draw[edge changed] (node-0-0) -- (node-1-0);
\draw[edge changed] (node-0-1) -- (node-1-1);
\draw[edge] (node-0-2) -- (node-0-3);
\draw[edge] (node-0-3) -- (node-0-4);
\draw[edge] (node-0-4) -- (node-0-5);
\draw[edge] (node-0-5) -- (node-0-6);
\draw[edge] (node-0-6) -- (node-0-7);
\draw[edge] (node-0-7) -- (node-0-8);
\draw[edge] (node-0-8) -- (node-0-9);
\draw[edge changed] (node-1-0) -- (node-1-1);
\draw[edge changed] (node-1-1) -- (node-1-2);
\draw[edge changed] (node-1-2) -- (node-2-2);
\draw[edge] (node-1-3) -- (node-2-3);
\draw[edge] (node-1-4) -- (node-1-5);
\draw[edge] (node-1-5) -- (node-1-6);
\draw[edge] (node-1-6) -- (node-2-6);
\draw[edge] (node-1-7) -- (node-1-8);
\draw[edge] (node-1-8) -- (node-2-8);
\draw[edge] (node-2-0) -- (node-3-0);
\draw[edge] (node-2-1) -- (node-3-1);
\draw[edge changed] (node-2-2) -- (node-3-2);
\draw[edge changed] (node-2-3) -- (node-3-3);
\draw[edge] (node-2-4) -- (node-2-5);
\draw[edge] (node-2-5) -- (node-2-6);
\draw[edge] (node-2-6) -- (node-2-7);
\draw[edge] (node-2-7) -- (node-2-8);
\draw[edge] (node-2-8) -- (node-2-9);
\draw[edge] (node-3-0) -- (node-3-1);
\draw[edge changed] (node-3-1) -- (node-3-2);
\draw[edge changed] (node-3-2) -- (node-3-3);
\draw[edge changed] (node-3-3) -- (node-4-3);
\draw[edge] (node-3-4) -- (node-4-4);
\draw[edge] (node-3-5) -- (node-4-5);
\draw[edge] (node-3-6) -- (node-3-7);
\draw[edge] (node-3-7) -- (node-4-7);
\draw[edge] (node-3-8) -- (node-4-8);
\draw[edge] (node-4-0) -- (node-5-0);
\draw[edge] (node-4-1) -- (node-5-1);
\draw[edge] (node-4-2) -- (node-5-2);
\draw[edge changed] (node-4-3) -- (node-4-4);
\draw[edge changed] (node-4-4) -- (node-5-4);
\draw[edge] (node-4-5) -- (node-5-5);
\draw[edge] (node-4-6) -- (node-5-6);
\draw[edge] (node-4-7) -- (node-5-7);
\draw[edge] (node-4-8) -- (node-5-8);
\draw[edge] (node-5-0) -- (node-6-0);
\draw[edge] (node-5-1) -- (node-6-1);
\draw[edge] (node-5-2) -- (node-6-2);
\draw[edge] (node-5-3) -- (node-6-3);
\draw[edge changed] (node-5-4) -- (node-5-5);
\draw[edge changed] (node-5-5) -- (node-6-5);
\draw[edge] (node-5-6) -- (node-5-7);
\draw[edge] (node-5-7) -- (node-5-8);
\draw[edge] (node-5-8) -- (node-5-9);
\draw[edge] (node-6-0) -- (node-7-0);
\draw[edge] (node-6-1) -- (node-7-1);
\draw[edge] (node-6-2) -- (node-7-2);
\draw[edge] (node-6-3) -- (node-7-3);
\draw[edge changed] (node-6-4) -- (node-6-5);
\draw[edge] (node-6-5) -- (node-7-5);
\draw[edge] (node-6-6) -- (node-6-7);
\draw[edge] (node-6-7) -- (node-6-8);
\draw[edge] (node-6-8) -- (node-7-8);
\draw[edge] (node-7-0) -- (node-8-0);
\draw[edge] (node-7-1) -- (node-8-1);
\draw[edge] (node-7-2) -- (node-7-3);
\draw[edge] (node-7-3) -- (node-8-3);
\draw[edge] (node-7-4) -- (node-8-4);
\draw[edge] (node-7-5) -- (node-8-5);
\draw[edge] (node-7-6) -- (node-8-6);
\draw[edge] (node-7-7) -- (node-7-8);
\draw[edge] (node-7-8) -- (node-7-9);
\draw[edge] (node-8-0) -- (node-9-0);
\draw[edge] (node-8-1) -- (node-9-1);
\draw[edge] (node-8-2) -- (node-9-2);
\draw[edge] (node-8-3) -- (node-9-3);
\draw[edge changed] (node-8-4) -- (node-8-5);
\draw[edge] (node-8-5) -- (node-9-5);
\draw[edge] (node-8-6) -- (node-9-6);
\draw[edge] (node-8-7) -- (node-9-7);
\draw[edge] (node-8-8) -- (node-8-9);
\node[highlight box] at (0.5,1.5) {};
\node[highlight box] at (2.5,3.5) {};
\node[highlight box] at (3.5,1.5) {};
\node[highlight box] at (5.5,5.5) {};


==> figures/autogenerated/rayleigh-spacing-content.tex <==
%% Auto-generated by rayleigh_spacing_tikz_export.py
%% (trees-SageMath: notebooks/probability/bifurcation-spacing/)
%% -- do not edit by hand.
% Input data: data/statistical_samples/geodesic_trees_n1000000.jsonl
% (Plancherel n=10^6 cusp forests, trees-SageMath).
% Nearest-neighbor spacings of the RAW directions z in [0,1]
% (no coordinate change), ensemble-unfolded: each point is mapped
% through the pooled empirical integrated density Nhat(z) =
% #{pooled points <= z}/M estimated from all M=2000 realizations
% (parameter-free); restricted to spacing midpoints in the bulk
% [0.10, 0.90]; pooled, rescaled to mean 1.
%% x=s (mean 1), y=density.
% n=10^6; 70970 spacings; pre-rescale pooled mean 1.000307;
% bin width 0.10; KS vs Rayleigh = 0.0023.
%% --- histogram bars (Monte Carlo data) ---
\fill[histbar] (0.000,0) rectangle (0.100,0.0831);
\fill[histbar] (0.100,0) rectangle (0.200,0.2273);
\fill[histbar] (0.200,0) rectangle (0.300,0.3762);
\fill[histbar] (0.300,0) rectangle (0.400,0.5037);
\fill[histbar] (0.400,0) rectangle (0.500,0.6021);
\fill[histbar] (0.500,0) rectangle (0.600,0.6711);
\fill[histbar] (0.600,0) rectangle (0.700,0.7324);
\fill[histbar] (0.700,0) rectangle (0.800,0.7366);
\fill[histbar] (0.800,0) rectangle (0.900,0.7664);
\fill[histbar] (0.900,0) rectangle (1.000,0.7383);
\fill[histbar] (1.000,0) rectangle (1.100,0.6814);
\fill[histbar] (1.100,0) rectangle (1.200,0.6425);
\fill[histbar] (1.200,0) rectangle (1.300,0.5890);
\fill[histbar] (1.300,0) rectangle (1.400,0.5089);
\fill[histbar] (1.400,0) rectangle (1.500,0.4295);
\fill[histbar] (1.500,0) rectangle (1.600,0.3724);
\fill[histbar] (1.600,0) rectangle (1.700,0.3039);
\fill[histbar] (1.700,0) rectangle (1.800,0.2474);
\fill[histbar] (1.800,0) rectangle (1.900,0.1980);
\fill[histbar] (1.900,0) rectangle (2.000,0.1625);
\fill[histbar] (2.000,0) rectangle (2.100,0.1219);
\fill[histbar] (2.100,0) rectangle (2.200,0.0931);
\fill[histbar] (2.200,0) rectangle (2.300,0.0607);
\fill[histbar] (2.300,0) rectangle (2.400,0.0445);
\fill[histbar] (2.400,0) rectangle (2.500,0.0307);
\fill[histbar] (2.500,0) rectangle (2.600,0.0213);
\fill[histbar] (2.600,0) rectangle (2.700,0.0207);
\fill[histbar] (2.700,0) rectangle (2.800,0.0130);
\fill[histbar] (2.800,0) rectangle (2.900,0.0079);
\fill[histbar] (2.900,0) rectangle (3.000,0.0051);
\fill[histbar] (3.000,0) rectangle (3.100,0.0028);
\fill[histbar] (3.100,0) rectangle (3.200,0.0018);
\fill[histbar] (3.200,0) rectangle (3.300,0.0013);
\fill[histbar] (3.300,0) rectangle (3.400,0.0008);
\fill[histbar] (3.400,0) rectangle (3.500,0.0003);
\fill[histbar] (3.500,0) rectangle (3.600,0.0006);
\fill[histbar] (3.600,0) rectangle (3.700,0.0000);
\fill[histbar] (3.700,0) rectangle (3.800,0.0001);
\fill[histbar] (3.800,0) rectangle (3.900,0.0000);
\fill[histbar] (3.900,0) rectangle (4.000,0.0003);
%% --- Rayleigh density P(s)=(pi/2) s exp(-pi s^2/4) ---
\draw[raycurve] plot coordinates {(0.000,0.0000) (0.010,0.0157) (0.020,0.0314) (0.030,0.0471) (0.040,0.0628) (0.050,0.0784) (0.060,0.0940) (0.070,0.1095) (0.080,0.1250) (0.090,0.1405) (0.100,0.1559) (0.110,0.1712) (0.120,0.1864) (0.130,0.2015) (0.140,0.2166) (0.150,0.2315) (0.160,0.2463) (0.170,0.2610) (0.180,0.2756) (0.190,0.2901) (0.200,0.3044) (0.210,0.3186) (0.220,0.3327) (0.230,0.3466) (0.240,0.3603) (0.250,0.3739) (0.260,0.3873) (0.270,0.4005) (0.280,0.4136) (0.290,0.4264) (0.300,0.4391) (0.310,0.4515) (0.320,0.4638) (0.330,0.4759) (0.340,0.4877) (0.350,0.4993) (0.360,0.5108) (0.370,0.5219) (0.380,0.5329) (0.390,0.5436) (0.400,0.5541) (0.410,0.5644) (0.420,0.5744) (0.430,0.5841) (0.440,0.5937) (0.450,0.6029) (0.460,0.6119) (0.470,0.6207) (0.480,0.6292) (0.490,0.6374) (0.500,0.6454) (0.510,0.6531) (0.520,0.6605) (0.530,0.6677) (0.540,0.6746) (0.550,0.6812) (0.560,0.6876) (0.570,0.6937) (0.580,0.6995) (0.590,0.7051) (0.600,0.7104) (0.610,0.7154) (0.620,0.7201) (0.630,0.7246) (0.640,0.7288) (0.650,0.7327) (0.660,0.7363) (0.670,0.7397) (0.680,0.7429) (0.690,0.7457) (0.700,0.7483) (0.710,0.7506) (0.720,0.7527) (0.730,0.7545) (0.740,0.7561) (0.750,0.7574) (0.760,0.7584) (0.770,0.7592) (0.780,0.7598) (0.790,0.7601) (0.800,0.7602) (0.810,0.7600) (0.820,0.7596) (0.830,0.7590) (0.840,0.7581) (0.850,0.7570) (0.860,0.7557) (0.870,0.7542) (0.880,0.7524) (0.890,0.7505) (0.900,0.7483) (0.910,0.7459) (0.920,0.7434) (0.930,0.7406) (0.940,0.7377) (0.950,0.7345) (0.960,0.7312) (0.970,0.7277) (0.980,0.7240) (0.990,0.7202) (1.000,0.7162) (1.010,0.7120) (1.020,0.7077) (1.030,0.7032) (1.040,0.6986) (1.050,0.6938) (1.060,0.6889) (1.070,0.6839) (1.080,0.6787) (1.090,0.6734) (1.100,0.6680) (1.110,0.6625) (1.120,0.6569) (1.130,0.6511) (1.140,0.6453) (1.150,0.6393) (1.160,0.6333) (1.170,0.6272) (1.180,0.6210) (1.190,0.6147) (1.200,0.6083) (1.210,0.6019) (1.220,0.5954) (1.230,0.5888) (1.240,0.5822) (1.250,0.5755) (1.260,0.5688) (1.270,0.5620) (1.280,0.5552) (1.290,0.5484) (1.300,0.5415) (1.310,0.5346) (1.320,0.5277) (1.330,0.5207) (1.340,0.5138) (1.350,0.5068) (1.360,0.4998) (1.370,0.4928) (1.380,0.4858) (1.390,0.4787) (1.400,0.4717) (1.410,0.4647) (1.420,0.4577) (1.430,0.4508) (1.440,0.4438) (1.450,0.4369) (1.460,0.4299) (1.470,0.4230) (1.480,0.4161) (1.490,0.4093) (1.500,0.4025) (1.510,0.3957) (1.520,0.3890) (1.530,0.3822) (1.540,0.3756) (1.550,0.3690) (1.560,0.3624) (1.570,0.3558) (1.580,0.3494) (1.590,0.3429) (1.600,0.3365) (1.610,0.3302) (1.620,0.3239) (1.630,0.3177) (1.640,0.3116) (1.650,0.3055) (1.660,0.2994) (1.670,0.2935) (1.680,0.2876) (1.690,0.2817) (1.700,0.2759) (1.710,0.2702) (1.720,0.2646) (1.730,0.2590) (1.740,0.2535) (1.750,0.2481) (1.760,0.2427) (1.770,0.2374) (1.780,0.2322) (1.790,0.2270) (1.800,0.2219) (1.810,0.2169) (1.820,0.2120) (1.830,0.2071) (1.840,0.2024) (1.850,0.1977) (1.860,0.1930) (1.870,0.1884) (1.880,0.1840) (1.890,0.1795) (1.900,0.1752) (1.910,0.1709) (1.920,0.1667) (1.930,0.1626) (1.940,0.1586) (1.950,0.1546) (1.960,0.1507) (1.970,0.1468) (1.980,0.1431) (1.990,0.1394) (2.000,0.1358) (2.010,0.1322) (2.020,0.1287) (2.030,0.1253) (2.040,0.1220) (2.050,0.1187) (2.060,0.1155) (2.070,0.1123) (2.080,0.1093) (2.090,0.1063) (2.100,0.1033) (2.110,0.1004) (2.120,0.0976) (2.130,0.0948) (2.140,0.0921) (2.150,0.0895) (2.160,0.0869) (2.170,0.0844) (2.180,0.0820) (2.190,0.0796) (2.200,0.0772) (2.210,0.0749) (2.220,0.0727) (2.230,0.0705) (2.240,0.0684) (2.250,0.0663) (2.260,0.0643) (2.270,0.0623) (2.280,0.0604) (2.290,0.0585) (2.300,0.0567) (2.310,0.0549) (2.320,0.0532) (2.330,0.0515) (2.340,0.0498) (2.350,0.0482) (2.360,0.0467) (2.370,0.0452) (2.380,0.0437) (2.390,0.0423) (2.400,0.0409) (2.410,0.0395) (2.420,0.0382) (2.430,0.0369) (2.440,0.0357) (2.450,0.0345) (2.460,0.0333) (2.470,0.0322) (2.480,0.0311) (2.490,0.0300) (2.500,0.0290) (2.510,0.0280) (2.520,0.0270) (2.530,0.0261) (2.540,0.0251) (2.550,0.0242) (2.560,0.0234) (2.570,0.0226) (2.580,0.0217) (2.590,0.0210) (2.600,0.0202) (2.610,0.0195) (2.620,0.0188) (2.630,0.0181) (2.640,0.0174) (2.650,0.0168) (2.660,0.0161) (2.670,0.0155) (2.680,0.0149) (2.690,0.0144) (2.700,0.0138) (2.710,0.0133) (2.720,0.0128) (2.730,0.0123) (2.740,0.0118) (2.750,0.0114) (2.760,0.0109) (2.770,0.0105) (2.780,0.0101) (2.790,0.0097) (2.800,0.0093) (2.810,0.0089) (2.820,0.0086) (2.830,0.0082) (2.840,0.0079) (2.850,0.0076) (2.860,0.0073) (2.870,0.0070) (2.880,0.0067) (2.890,0.0064) (2.900,0.0062) (2.910,0.0059) (2.920,0.0057) (2.930,0.0054) (2.940,0.0052) (2.950,0.0050) (2.960,0.0048) (2.970,0.0046) (2.980,0.0044) (2.990,0.0042) (3.000,0.0040) (3.010,0.0038) (3.020,0.0037) (3.030,0.0035) (3.040,0.0034) (3.050,0.0032) (3.060,0.0031) (3.070,0.0029) (3.080,0.0028) (3.090,0.0027) (3.100,0.0026) (3.110,0.0025) (3.120,0.0023) (3.130,0.0022) (3.140,0.0021) (3.150,0.0020) (3.160,0.0019) (3.170,0.0019) (3.180,0.0018) (3.190,0.0017) (3.200,0.0016) (3.210,0.0015) (3.220,0.0015) (3.230,0.0014) (3.240,0.0013) (3.250,0.0013) (3.260,0.0012) (3.270,0.0012) (3.280,0.0011) (3.290,0.0011) (3.300,0.0010) (3.310,0.0010) (3.320,0.0009) (3.330,0.0009) (3.340,0.0008) (3.350,0.0008) (3.360,0.0007) (3.370,0.0007) (3.380,0.0007) (3.390,0.0006) (3.400,0.0006) (3.410,0.0006) (3.420,0.0006) (3.430,0.0005) (3.440,0.0005) (3.450,0.0005) (3.460,0.0004) (3.470,0.0004) (3.480,0.0004) (3.490,0.0004) (3.500,0.0004) (3.510,0.0003) (3.520,0.0003) (3.530,0.0003) (3.540,0.0003) (3.550,0.0003) (3.560,0.0003) (3.570,0.0003) (3.580,0.0002) (3.590,0.0002) (3.600,0.0002) (3.610,0.0002) (3.620,0.0002) (3.630,0.0002) (3.640,0.0002) (3.650,0.0002) (3.660,0.0002) (3.670,0.0001) (3.680,0.0001) (3.690,0.0001) (3.700,0.0001) (3.710,0.0001) (3.720,0.0001) (3.730,0.0001) (3.740,0.0001) (3.750,0.0001) (3.760,0.0001) (3.770,0.0001) (3.780,0.0001) (3.790,0.0001) (3.800,0.0001) (3.810,0.0001) (3.820,0.0001) (3.830,0.0001) (3.840,0.0001) (3.850,0.0001) (3.860,0.0001) (3.870,0.0000) (3.880,0.0000) (3.890,0.0000) (3.900,0.0000) (3.910,0.0000) (3.920,0.0000) (3.930,0.0000) (3.940,0.0000) (3.950,0.0000) (3.960,0.0000) (3.970,0.0000) (3.980,0.0000) (3.990,0.0000) (4.000,0.0000)};
%% --- exponential null P(s)=exp(-s) ---
\draw[expcurve] plot coordinates {(0.000,1.0000) (0.010,0.9900) (0.020,0.9802) (0.030,0.9704) (0.040,0.9608) (0.050,0.9512) (0.060,0.9418) (0.070,0.9324) (0.080,0.9231) (0.090,0.9139) (0.100,0.9048) (0.110,0.8958) (0.120,0.8869) (0.130,0.8781) (0.140,0.8694) (0.150,0.8607) (0.160,0.8521) (0.170,0.8437) (0.180,0.8353) (0.190,0.8270) (0.200,0.8187) (0.210,0.8106) (0.220,0.8025) (0.230,0.7945) (0.240,0.7866) (0.250,0.7788) (0.260,0.7711) (0.270,0.7634) (0.280,0.7558) (0.290,0.7483) (0.300,0.7408) (0.310,0.7334) (0.320,0.7261) (0.330,0.7189) (0.340,0.7118) (0.350,0.7047) (0.360,0.6977) (0.370,0.6907) (0.380,0.6839) (0.390,0.6771) (0.400,0.6703) (0.410,0.6637) (0.420,0.6570) (0.430,0.6505) (0.440,0.6440) (0.450,0.6376) (0.460,0.6313) (0.470,0.6250) (0.480,0.6188) (0.490,0.6126) (0.500,0.6065) (0.510,0.6005) (0.520,0.5945) (0.530,0.5886) (0.540,0.5827) (0.550,0.5769) (0.560,0.5712) (0.570,0.5655) (0.580,0.5599) (0.590,0.5543) (0.600,0.5488) (0.610,0.5434) (0.620,0.5379) (0.630,0.5326) (0.640,0.5273) (0.650,0.5220) (0.660,0.5169) (0.670,0.5117) (0.680,0.5066) (0.690,0.5016) (0.700,0.4966) (0.710,0.4916) (0.720,0.4868) (0.730,0.4819) (0.740,0.4771) (0.750,0.4724) (0.760,0.4677) (0.770,0.4630) (0.780,0.4584) (0.790,0.4538) (0.800,0.4493) (0.810,0.4449) (0.820,0.4404) (0.830,0.4360) (0.840,0.4317) (0.850,0.4274) (0.860,0.4232) (0.870,0.4190) (0.880,0.4148) (0.890,0.4107) (0.900,0.4066) (0.910,0.4025) (0.920,0.3985) (0.930,0.3946) (0.940,0.3906) (0.950,0.3867) (0.960,0.3829) (0.970,0.3791) (0.980,0.3753) (0.990,0.3716) (1.000,0.3679) (1.010,0.3642) (1.020,0.3606) (1.030,0.3570) (1.040,0.3535) (1.050,0.3499) (1.060,0.3465) (1.070,0.3430) (1.080,0.3396) (1.090,0.3362) (1.100,0.3329) (1.110,0.3296) (1.120,0.3263) (1.130,0.3230) (1.140,0.3198) (1.150,0.3166) (1.160,0.3135) (1.170,0.3104) (1.180,0.3073) (1.190,0.3042) (1.200,0.3012) (1.210,0.2982) (1.220,0.2952) (1.230,0.2923) (1.240,0.2894) (1.250,0.2865) (1.260,0.2837) (1.270,0.2808) (1.280,0.2780) (1.290,0.2753) (1.300,0.2725) (1.310,0.2698) (1.320,0.2671) (1.330,0.2645) (1.340,0.2618) (1.350,0.2592) (1.360,0.2567) (1.370,0.2541) (1.380,0.2516) (1.390,0.2491) (1.400,0.2466) (1.410,0.2441) (1.420,0.2417) (1.430,0.2393) (1.440,0.2369) (1.450,0.2346) (1.460,0.2322) (1.470,0.2299) (1.480,0.2276) (1.490,0.2254) (1.500,0.2231) (1.510,0.2209) (1.520,0.2187) (1.530,0.2165) (1.540,0.2144) (1.550,0.2122) (1.560,0.2101) (1.570,0.2080) (1.580,0.2060) (1.590,0.2039) (1.600,0.2019) (1.610,0.1999) (1.620,0.1979) (1.630,0.1959) (1.640,0.1940) (1.650,0.1920) (1.660,0.1901) (1.670,0.1882) (1.680,0.1864) (1.690,0.1845) (1.700,0.1827) (1.710,0.1809) (1.720,0.1791) (1.730,0.1773) (1.740,0.1755) (1.750,0.1738) (1.760,0.1720) (1.770,0.1703) (1.780,0.1686) (1.790,0.1670) (1.800,0.1653) (1.810,0.1637) (1.820,0.1620) (1.830,0.1604) (1.840,0.1588) (1.850,0.1572) (1.860,0.1557) (1.870,0.1541) (1.880,0.1526) (1.890,0.1511) (1.900,0.1496) (1.910,0.1481) (1.920,0.1466) (1.930,0.1451) (1.940,0.1437) (1.950,0.1423) (1.960,0.1409) (1.970,0.1395) (1.980,0.1381) (1.990,0.1367) (2.000,0.1353) (2.010,0.1340) (2.020,0.1327) (2.030,0.1313) (2.040,0.1300) (2.050,0.1287) (2.060,0.1275) (2.070,0.1262) (2.080,0.1249) (2.090,0.1237) (2.100,0.1225) (2.110,0.1212) (2.120,0.1200) (2.130,0.1188) (2.140,0.1177) (2.150,0.1165) (2.160,0.1153) (2.170,0.1142) (2.180,0.1130) (2.190,0.1119) (2.200,0.1108) (2.210,0.1097) (2.220,0.1086) (2.230,0.1075) (2.240,0.1065) (2.250,0.1054) (2.260,0.1044) (2.270,0.1033) (2.280,0.1023) (2.290,0.1013) (2.300,0.1003) (2.310,0.0993) (2.320,0.0983) (2.330,0.0973) (2.340,0.0963) (2.350,0.0954) (2.360,0.0944) (2.370,0.0935) (2.380,0.0926) (2.390,0.0916) (2.400,0.0907) (2.410,0.0898) (2.420,0.0889) (2.430,0.0880) (2.440,0.0872) (2.450,0.0863) (2.460,0.0854) (2.470,0.0846) (2.480,0.0837) (2.490,0.0829) (2.500,0.0821) (2.510,0.0813) (2.520,0.0805) (2.530,0.0797) (2.540,0.0789) (2.550,0.0781) (2.560,0.0773) (2.570,0.0765) (2.580,0.0758) (2.590,0.0750) (2.600,0.0743) (2.610,0.0735) (2.620,0.0728) (2.630,0.0721) (2.640,0.0714) (2.650,0.0707) (2.660,0.0699) (2.670,0.0693) (2.680,0.0686) (2.690,0.0679) (2.700,0.0672) (2.710,0.0665) (2.720,0.0659) (2.730,0.0652) (2.740,0.0646) (2.750,0.0639) (2.760,0.0633) (2.770,0.0627) (2.780,0.0620) (2.790,0.0614) (2.800,0.0608) (2.810,0.0602) (2.820,0.0596) (2.830,0.0590) (2.840,0.0584) (2.850,0.0578) (2.860,0.0573) (2.870,0.0567) (2.880,0.0561) (2.890,0.0556) (2.900,0.0550) (2.910,0.0545) (2.920,0.0539) (2.930,0.0534) (2.940,0.0529) (2.950,0.0523) (2.960,0.0518) (2.970,0.0513) (2.980,0.0508) (2.990,0.0503) (3.000,0.0498) (3.010,0.0493) (3.020,0.0488) (3.030,0.0483) (3.040,0.0478) (3.050,0.0474) (3.060,0.0469) (3.070,0.0464) (3.080,0.0460) (3.090,0.0455) (3.100,0.0450) (3.110,0.0446) (3.120,0.0442) (3.130,0.0437) (3.140,0.0433) (3.150,0.0429) (3.160,0.0424) (3.170,0.0420) (3.180,0.0416) (3.190,0.0412) (3.200,0.0408) (3.210,0.0404) (3.220,0.0400) (3.230,0.0396) (3.240,0.0392) (3.250,0.0388) (3.260,0.0384) (3.270,0.0380) (3.280,0.0376) (3.290,0.0373) (3.300,0.0369) (3.310,0.0365) (3.320,0.0362) (3.330,0.0358) (3.340,0.0354) (3.350,0.0351) (3.360,0.0347) (3.370,0.0344) (3.380,0.0340) (3.390,0.0337) (3.400,0.0334) (3.410,0.0330) (3.420,0.0327) (3.430,0.0324) (3.440,0.0321) (3.450,0.0317) (3.460,0.0314) (3.470,0.0311) (3.480,0.0308) (3.490,0.0305) (3.500,0.0302) (3.510,0.0299) (3.520,0.0296) (3.530,0.0293) (3.540,0.0290) (3.550,0.0287) (3.560,0.0284) (3.570,0.0282) (3.580,0.0279) (3.590,0.0276) (3.600,0.0273) (3.610,0.0271) (3.620,0.0268) (3.630,0.0265) (3.640,0.0263) (3.650,0.0260) (3.660,0.0257) (3.670,0.0255) (3.680,0.0252) (3.690,0.0250) (3.700,0.0247) (3.710,0.0245) (3.720,0.0242) (3.730,0.0240) (3.740,0.0238) (3.750,0.0235) (3.760,0.0233) (3.770,0.0231) (3.780,0.0228) (3.790,0.0226) (3.800,0.0224) (3.810,0.0221) (3.820,0.0219) (3.830,0.0217) (3.840,0.0215) (3.850,0.0213) (3.860,0.0211) (3.870,0.0209) (3.880,0.0207) (3.890,0.0204) (3.900,0.0202) (3.910,0.0200) (3.920,0.0198) (3.930,0.0196) (3.940,0.0194) (3.950,0.0193) (3.960,0.0191) (3.970,0.0189) (3.980,0.0187) (3.990,0.0185) (4.000,0.0183)};

